KRISM --- Krylov Subspace-based Optical Computing of Hyperspectral Images

We present an adaptive imaging technique that optically computes a low-rank approximation of a scene's hyperspectral image, conceptualized as a matrix. Central to the proposed technique is the optical implementation of two measurement operators: a spectrally-coded imager and a spatially-coded spectrometer. By iterating between the two operators, we show that the top singular vectors and singular values of a hyperspectral image can be adaptively and optically computed with only a few iterations. We present an optical design that uses pupil plane coding for implementing the two operations and show several compelling results using a lab prototype to demonstrate the effectiveness of the proposed hyperspectral imager.

==> limitations.tex <==
While our method promises fast acquisition times, it has the following disadvantages:
\begin{itemize}[leftmargin=*]
	\item \textbf{Complexity of optical setup} Our method requires an optical setup which can obtain spectrally coded images as well as spatially coded spectrum. Such an equipment has various problems such as light throughput, precise alignment,  and calibration across sensors, and hence can be tricky to build in a lab setting. However, such a drawback exists with any hyperspectral imaging setup and hence is not a serious drawback.
	%
	\item \textbf{Effectiveness at low spectral resolution} Our method is only advantageous if there are sufficient spectral bands and the hyperspectral image is sufficently low rank. If there are only a few spectral bands or the rank is significantly high, our method is as fast or slow as traditional sensing methods.
	%
	However, as we stated earlier, hyperspectral images are low rank, and hence this disadvantage is not a major concern.
\end{itemize}

==> method.tex <==
Consider a hyperspectral image $I$ with $N_1\times N_2$ spatial dimension and $N_3$ spectral bands. Let $X\in \rdim{N_3 \times  N_1 N_2}$ be matrix representation of the hyperspectral image with each row representing spectrum at each pixel. 
%
Hence, $\bfy = X\bfx$ is spatially coded spectrum and $\bfy = X^\top \bfx$ is spectrally coded image
%
Instead of having access to the elements of $X$, we have access to functions $\mathcal{F}$ and $\mathcal{A}$ such that,
\begin{align}
	\bfy &= \mathcal{F}(\bfx) = X\bfx +\bfe \quad \textrm{and},\nonumber\\
	\bfy^\prime &= \mathcal{A}(\bfx^\prime) = X^\top \bfx^\prime + \bfe^\prime.
\end{align}
%
Our goal is to obtain top $k$ eigenvectors of $X$, given an optical setup that can only obtain spectrally coded images or spatially coded spectrum. 
%
We outline the steps involved in Algorithm \ref{alg:ohs}
\input{optical_hs.tex}

After $L$ iterations, we obtain the leading spatial and spectral eigenvectors and the singular values, thus giving a highly accurate estimate of the hyperspectral image.
%
In practise, we use the Arnoldi method, which performs power iterations with a single vector in each step instead of $k$ vectors. While both are equivalent, we show all our proofs with the subspace iteration method and show simulation results with the Arnoldi method.

\subsection{Performance comparison}
Table \ref{tab:meas_comp} compares various sensing strategies against our proposed method. Derivations of expressions can be found in the supplementary material.
%
Amongst all the methods, our method computes highly accurate subspace estimate with the fewest number of measurements. 
%
Specifically, compared to CS, our method requires a factor of $k$ fewer measurements for accurate estimate of a rank-$k$ subspace. 
%
Without any doubt, it outperforms any other method by a large margin in terms of number of measurements.

Comparison of noise performance is a bit tricky, as our method estimates a subspace instead of the complete cube.
%
Noise performance is the same compared to CS with row/column projection.
%
There is an improved performance over sampling based techniques but not necessarily over multiplexed methods.

There is definitely a small price to pay for such gains. First, the optical setup is complex compared to all other methods.
%
While other methods either require spatial/spectral scanning or spatial/spectral multiplexing, we need a joint spatial \textit{and} spectral coding.
%
Secondly, since our method is adaptive, there is an overhead of computational time.
%
In spite of this overhead, we show in our real experiments that the time of acquisition and quality of reconstruction is far superior than any other method.


==> notation.tex <==
We denote vectors in bold font, scalars in small letters and matrices in capital letters. 
%
Let $\mathcal{X}\in \mathbb{R}^{N_x \times N_y \times N_\lambda}$ be a hyperspectral image with $N_x \times N_y$ spatial resolution and $N_\lambda$ spectral bands.
%
Then, $X \in \mathbb{R}^{N_xN_y\times N_\lambda}$ is the matrix representation of $\mathcal{X}$, where each column is an image and each row is a spectrum.

==> npm.tex <==
% Noisy power method

\begin{algorithm}[h]
	\caption{Noisy Power Method}
	\label{alg:npm}
	\begin{algorithmic}
		\Require Symmetric matrix $X\in \rdim{n\times n}$, Number of iterations $L$, dimension $k$
		\State Start with $X_0 \in \rdim{n\times p}$
		
		\For{$l = 1$ to $L$}
			\State $Y_l \leftarrow AX_{l-1} + E_l$ \Comment{(Matrix vectors multiplication)}
			\State $(X_l, R_l) \leftarrow \textrm{QR}(Y_l)$ \Comment{(QR Factorization)}
		\EndFor
		
		\State \Return $X_L$
	\end{algorithmic}
\end{algorithm}

==> nsvd.tex <==
% Noisy power method

\begin{algorithm}[h]
	\caption{Noisy SVD, adopted from \cite{str-6}}
	\label{alg:nsvd}
	\begin{algorithmic}
		\Require Matrix $X\in \rdim{m\times n}$, Number of iterations $L$, dimension $k$
		\State Start with $q_0 \in \rdim{n\times 1} such that $\|q_0\| = 1$
		
		\For{$j = 1$ to $L$}
			\State P_{j-1} = [p_1, p2, \cdots, p_{j-1}]
			\State $p_l \leftarrow Xq_l$ 
			\State Orthogonalize $p_j$ w.r.t P_{j-1}
			\State \alpha_j \|p_j\|_2
			\State p_j = p_j/\alpha_j
			\State 
		\EndFor
		
		\State \Return $X_L$
	\end{algorithmic}
\end{algorithm}

==> oc_code_design.tex <==
Ideally, we want to achieve spectral measurements $s_\text{slit}(x, y)$ and spatial measurements $I_{3, \text{open}}$
%
Equations \ref{eq:spec} and \ref{eq:im} encapsulate the effect of an aperture pattern on spectral resolution as well as spatial resolution. 
%
From previous sections, it is clear that neither a slit or a fully open aperture enables high resolution imaging.

The required change in philosophy is the following: \emph{Provided we can reverse the effect of an aperture code on spectral and spatial measurements, we can achieve high resolution hyperspectral imaging}
%
The natural extension to this statement is, \textbf{what are good aperture codes $a(x)$ such that the spectrum can be deconvolved with this code, \emph{and} the spatial image can be deconvolved with the power spectral density of the code?}

To narrow our definition further, we define invertible codes as those which have no nulls in frequency space, thus promising complete recovery of original data.
%
Putting it more concretely, $a(x)$ must have no nulls in frequency space \emph{and} $C_a(x)$ must have no nulls in frequency space. 
%
Provided $a(x)$ satisfies those conditions, we can achieve simultaneous high spatio-spectral resolution.
% 
However, under noisy measurement conditions, simply having no nulls will not suffice; the noise might get amplified anywhere the frequency response is too low.
%
The objetive function then becomes clear -- \emph{To simultaneously maximize the minimum spectrum value of $a(x)$ and $C_a(x)$}. 

\subsection{Optimal binary codes}
Since manufacturing of binary codes is the easiest, we stick to design of finite sized binary aperture codes.
%
The specific form of our binary codes is:
\begin{align}
	a(x) &= \sum\limits_{k=0}^{N-1} a_k \mathbb{I}_{[kh, (k+1)h]}(x),
\end{align}
where $\mathbb{I}_{[kh, (k+1)h]}(x) = 1 \forall x \in [kh, (k+1)h]$. Let $A=\{a_k\}$ be the required binary code.
%
This representation captures finite binary codes with non-zero width of $h$ units per each bit.

If we optimize for $a(x)$ alone, then the answer is $\delta(x)$. Similarly, optimizing for $C_a(x)$ alone gives us $a(x) = 1$. This means that $a(x)$ and $C_a(x)$ have opposing effects; Maximizing minimum value of spectrum of $a(x)$ works against $C_a(x)$ and vice versa.
%
Hence we propose the following intuitive compound  objective:
\begin{align}
	& \max_{A} &&\alpha \min_u \left(|\mathcal{F}(a)(u)|\right) + (1-\alpha ) \min_u \left(|\mathcal{F}(C_a)(u)|\right)
	\label{eq:obj_opt}\\
	& \text{Subject to}	 && A \in \{0, 1\}^N,\nonumber
\end{align}

where $\alpha \in (0, 1)$ is a constant. We have not explored the nature of objective function (\ref{eq:obj_opt}) but do believe it is combinatorial in nature, which makes it extremely hard to minimize.
%
Fortunately, our code lengths $N$ are smaller than $32$, which means that we can brute force a solution.

\subsection{Optimal imperceptible codes}
Instead of having invertible spectral and invertible spatial codes, we can have invertible spectral code such that the spatial blur is imperceptible. 
%
In this case, we minimize the ratio of first two peaks of the spatial blur point spread function (PSF).
%
Let $P_a(x)$ be the spatial PSF created by $a(x)$. Let $\eta_1, \eta_2$ be the first and second maximum peak heights of $P_a(x)$. Then the objective function is:
%
\begin{align}
& \max_{A} &&\alpha \min_u \left(|\mathcal{F}(a)(u)|\right) + (1-\alpha )  \left(\frac{\eta_2}{\eta_1}\right)
\label{eq:obj_imperceptible}\\
& \text{Subject to}	 && A \in \{0, 1\}^N.\nonumber
\end{align}
As before, this objective function is combinatorial in nature. However we can brute force solutions for small sized codes.

==> oc_model.tex <==

\begin{figure}[!ttt]
	\centering
	\includegraphics[width=\columnwidth]{figures/4f.png}
	\caption{A $4f$ system diagram.}
	\label{fig:4f}
\end{figure}

Consider a simple $4f$ system shown in Fig. \ref{fig:4f}, where the first lens is kept a $f$ units away from the object plane $p_1$, the second lens is palced $2f$ units away from first lens and finally, the image is formed $f$ units after the second lens at $p_3$.
%
The plane $p_3$ then is the aperture plane, from a ray optics perspective. From a wave optics perspective, it is the scaled Fourier transform of the object plane $p_1$.

Let $f_1(x, y, \lambda)$ be the field at plane $p_1$. Then the field at $p_2$ is the scaled fourier transform, $f_2(x, y, \lambda) = F_1\left(\frac{x}{\lambda f}, \frac{y}{\lambda f}, \lambda\right)$, where $F_1(u, v, \lambda)$ is the 2D-Fourier transform of $f_1(x, y, \lambda)$.
%
By the same expression, the field at $p_3$ is then $f_3(x, y,\lambda) = f_1(-x, -y,\lambda)$, simply the inverted image.

\subsection{Spatio-spectral measurements}
%
\begin{figure*}[!ttt]
	\centering
	\includegraphics[width=\textwidth]{figures/spatio_spectrum.png}
	\caption{A $4f$ system with simultaneous spatial and spectral measurements. Aperture code decides the spatial and spectral resolution. Design of optimal binary codes for aperture can enable both high spatial and high spectral resolutions.}
	\label{fig:spatio_spec}
\end{figure*}
%
Now consider another setup shown in Fig. \ref{fig:spatio_spec}. We place a diffraction grating at the second image plane, which creates a wavelength-dependent shift of the aperture plane.
%
We measure spectral intensity $s(x, y)$ and image intensity $I_3(x, y)$ as shown in the figure.
%
We also add an aperture coded $a(x, y)$ before diffraction grating -- this helps us analyze the effect of coded aperture on spectral and/or spatial blurring.
%
Note that off-the-shelf objective lenses can also be treated as $4f$ systems and hence the analysis stays the same.

Assuming that the light from plane $p_1$ is incoherent. The field just before the aperture code is $f_2(x, y, \lambda) = F_1\left(\frac{x}{\lambda f}, \frac{y}{\lambda f}, \lambda\right)$.
%
Then, the field just after the aperture code is $\hat{f}_2(x, y, \lambda) = a(x, y)\cdot f_2(x, y, \lambda)$. Then the intensity image on diffraction grating,
\begin{align}
	I_3(x, y, \lambda) &= |\hat{F}_2\left(\frac{x}{\lambda f}, \frac{y}{\lambda f}, \lambda \right)|^2\nonumber\\
	          &= I_1(-x, -y, \lambda) \ast C_a \left(\frac{x}{\lambda f}, \frac{y}{\lambda f}\right),
\end{align}
where $C_a(x, y)$ is the linear autocorrelation of $a(x, y)$ and $\ast$ represenents linear convolution.
%
Since all wavelengths recombine after $4f$ units, the final intensity image is $I_3(x, y)$.
%
Recollect that the diffraction grading does a wavelength dependent shift of aperture field. Assuming that the grating splits wavelengths along x-axis, we have,
\begin{align}
	s(x, y) &= \int_{\lambda=-\infty}^{\infty} \hat{f}_2(x - c \lambda, y, \lambda) d\lambda\nonumber\\
            &= \int_{\lambda=-\infty}^{\infty} f_2(x - c \lambda, y, \lambda) a(x - c \lambda, y) d\lambda,\\
    I_3(x, y) 	&= \int_{\lambda=-\infty}^{\infty} I_3(x, y, \lambda) d\lambda
\end{align}

\subsection{Case 1: Ideal slit along y-axis}

In this case, we have, $a(x, y) = \delta(x)$. Hence the spectral intensity,
\begin{align}
	s_\text{slit}(x, y) &= \int_{\lambda=-\infty}^{\infty} f_2(x - c \lambda, y, \lambda) a(x - c \lambda, y) d\lambda\nonumber\\
	 			  &= \int_{\lambda=-\infty}^{\infty} f_2(x - c \lambda, y, \lambda) \delta(x - c \lambda) d\lambda\nonumber\\
	 			  &= f_2(x - c x/c, y, x/c)\nonumber\\
	 			  &= f_2(0, y, \frac{x}{c}).
\end{align}
The spatial intensity,
\begin{align}
	I_{3,\text{slit}}(x, y) 	&= \int_{\lambda=-\infty}^{\infty} I_3(x, y, \lambda) d\lambda\nonumber \\
				&= \int_{\lambda=-\infty}^{\infty} I_1(-x, -y, \lambda) \ast C_a \left(\frac{x}{\lambda f}, \frac{y}{\lambda f} \right) d\lambda\nonumber\\
 	C_a \left(x, y \right) &= \mathcal{F}_{2D}(\delta(x))\nonumber\\
 	 					   &= \delta(y)\nonumber\\
   \implies I_{3,\text{slit}}(x, y) 	&=\int_{\lambda=-\infty}^{\infty} I_1(-x, -y, \lambda) \ast \delta \left( \frac{y}{\lambda f} \right) d\lambda\nonumber\\
   						&= \int_{\lambda=-\infty}^{\infty} \int_{\xi=-\infty}^{\infty} I_1(-\xi, -y, \lambda) d\xi d\lambda,
\end{align}
which results in a completely blurred image along x-axis. 

\subsection{Case 2: Ideal open aperture}

In this case, we have, $a(x, y) = 1$. Evaluating expressions as before, we get,
\begin{align}
	s_\text{open} (x, y) &= \int\limits_{\lambda=-\infty}^{\infty} f_2(x - c \lambda, y, \lambda) d\lambda\\
	I_{3,\text{open}} (x, y) &= \int_{\lambda=-\infty}^{\infty} I_1(-x, -y, \lambda) d\lambda.
\end{align}
This results in a very sharp intensity image but a completely blurred spectrum, opposite of the previous case. Unfortunately, neither is appealing to high resolution hyperspectral imaging.

Before we discuss design of optimal codes, we do a modification of our system. Recall that spectral blur only happens along x-axis. Hence, y-axis can be trivially left completely open. This means that the code can be $a(x, y) = a(x)$ and there will be no loss of resolution. With this, our measurement expressions become:
%
\begin{align}
s(x, y) &= \int_{\lambda=-\infty}^{\infty} f_2(x - c \lambda, y, \lambda) a(x - c \lambda) d\lambda,\\
I_3(x, y) 	&= \int_{\lambda=-\infty}^{\infty} I_1(-x, -y, \lambda) \ast C_a\left( \frac{x}{\lambda f}\right) d\lambda.
\end{align}
%
This leads to another simplification in analysis. Since the y-axis is untouched in either spectral or spatial measurements, we can simply ignore it and analyze just x-axis, giving us,
%
\begin{align}
s(x) &= \int_{\lambda=-\infty}^{\infty} f_2(x - c \lambda, \lambda) a(x - c \lambda) d\lambda,\\
I_3(x) 	&= \int_{\lambda=-\infty}^{\infty} I_1(-x, \lambda) \ast C_a\left( \frac{x}{\lambda f}\right) \label{eq:im}d\lambda.
\end{align}
%
Finally, assuming $f_2(x, \lambda)$ is approximately constant over the aperture area, we have,
\begin{align}
s(x) &= \int_{\lambda=-\infty}^{\infty} f_2(0, \lambda) a(x - c \lambda) d\lambda,\nonumber\\
	 &= f_2(0, x) \ast a(x)\label{eq:spec}
\end{align}

==> oc_synthetic.tex <==
\subsection{Invertible vs imperceptible codes}
\begin{figure}[!ttt]
	\centering
	\begin{subfigure}[t]{\columnwidth}
		\centering
		\includegraphics[width=0.45\textwidth]{figures/synthetic/aperture_29_invertible}
		\quad
		\includegraphics[width=0.45\textwidth]{figures/synthetic/synthetic_optn_29_raw.png}
		\caption{Invertible 29 dimensional code}
	\end{subfigure}
	\begin{subfigure}[t]{\columnwidth}
		\centering
		\includegraphics[width=0.45\textwidth]{figures/synthetic/aperture_31_imperceptible.png}
		\quad
		\includegraphics[width=0.45\textwidth]{figures/synthetic/synthetic_optm_31.png}
		\caption{Imperceptible 31 dimensional code.}
	\end{subfigure}
	\caption{Binary code and measured image for an invertible example and an imperceptible example. Imperceptible codes offer blur that is not visible, thus not requiring any image deconvolution.}
	\label{fig:code_compare}
\end{figure}
Invertible codes ensure that the resultant data can be easily deconvolved. On the other hand, imperceptible codes ensure that the spatial blur is not visible, thus removing the deconvolution step.
%
Depending on whether spatial information is important or spectral, one of the two codes is a better choice.
%
While both codes are reliable, the deconvolution process means that noise will be amplified.
%
When using invertible codes, the noise in image is amplified, whereas when using imperceptible codes, the noise in spectrum is amplified.
%
Noise in images can be reduced using TV-regularized deconvolution. Noise in spectrum can be reduced using smoothness priors. 
%
Hence the choice between the two classes depends on the design requirements.
%
Figure \ref{fig:code_compare} shows an example 29 dimensional invertible code and a 31 dimensional imperceptible code and the respective images.
%
The blur with imperceptible code is barely visible, which makes it an optimal choice for high-resolution image measurements.

\subsection{Performance of coded apertures}
\begin{figure}[!ttt]
	\centering
	\begin{subfigure}[t]{\columnwidth}
		\centering
		\includegraphics[width=0.45\textwidth]{figures/synthetic/synthetic_spec_31_iimperceptible_raw.pdf}
		\quad
		\includegraphics[width=0.45\textwidth]{figures/synthetic/synthetic_optm_31_raw.png}
		\caption{Raw measurements.}
	\end{subfigure}
	\begin{subfigure}[t]{\columnwidth}
		\centering
		\includegraphics[width=0.45\textwidth]{figures/synthetic/synthetic_spec_31_imperceptible.pdf}
		\quad
		\includegraphics[width=0.45\textwidth]{figures/synthetic/synthetic_optm_31.png}
		\caption{Deconvolved spectrum and image respectively.}
	\end{subfigure}
	\caption{Raw measurements and deconvolved Spectrum and spatial measurements respectively with optimally imperceptible codes of length 31. With optimal codes, we can obtain high spatial as well as spectral resolution.}
	\label{fig:optn_29}
\end{figure}

Figure \ref{fig:optn_29} shows deconvolved spectrum and deconvolved image with an optimally invertible code of length 29.
%
 Measurements were simulated with 30dB noise level. Weiner deconvolution was used for both spectrum and space.
%
Notice how the noise is fairly well suppressed in spectrum but shows up in the deconvolved spatial image.

==> optical_hs.tex <==
% OMP algorithm

\begin{algorithm}[h]
	\caption{Optical power method for hyperspectral imaging}
	\label{alg:ohs}
	\begin{algorithmic}
		\Require Function handles $\mathcal{F}()$ and $\mathcal{A}()$, subspace dimension $k$ and number of iterations $L$.
		\State Start with $X_0 \in \rdim{N_1 N_2\times k}$
		
		\For{$l = 1$ to $L$}
			\State $Y_l \leftarrow \mathcal{F}(X_{l-1}) + E_l$ \Comment{(Spatial coding)}
			\State $(\Lambda_l, R_l) \leftarrow \textrm{QR}(Y_l)$ \Comment{(QR Factorization)}
			\State $Y^\prime_l \leftarrow \mathcal{A}(\Lambda_l) + E^\prime_l$ \Comment{(Spectral coding)}
			\State $(X_l, R^\prime_l) \leftarrow \textrm{QR}(Y^\prime_l)$ \Comment{(QR Factorization)}
		\EndFor
		
		\State $S_L \leftarrow \textrm{diag}(R^\prime_L)$ 	\Comment{(Matrix with only diagonal elements)}
		\State \Return $X_L,S_L,\Lambda_L$
	\end{algorithmic}
\end{algorithm}

==> optics.tex <==
% Optics here

Our optical setup consists main of two components -- 1) Imaging with spectral coding and 2) Spectrum measurements of coded image. 

% And then explain everything else.

==> optimal_code.tex <==
\label{section:code}
%
\begin{figure*}[!ttt]
	\centering
	\begin{subfigure}[t]{0.35\columnwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{figures/synthetic/slit.png}
		\caption*{}
		\includegraphics[width=\textwidth]{figures/synthetic/slit_space.png}
		\caption*{}
		\includegraphics[height=1in]{figures/synthetic/slit_spectrum.pdf}
		\caption{Slit}
	\end{subfigure}
	\quad
	\begin{subfigure}[t]{0.35\columnwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{figures/synthetic/open_9.png}
		\caption*{}
		\includegraphics[width=\textwidth]{figures/synthetic/open_9_space.png}
		\caption*{}
		\includegraphics[height=1in]{figures/synthetic/open_9_spectrum.pdf}
		\caption{Small open aperture}
	\end{subfigure}
	\quad
	\begin{subfigure}[t]{0.35\columnwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{figures/synthetic/open_29.png}
		\caption*{}
		\includegraphics[width=\textwidth]{figures/synthetic/open_29_space.png}
		\caption*{}
		\includegraphics[height=1in]{figures/synthetic/open_29_spectrum.pdf}
		\caption{Large open aperture}
	\end{subfigure}
	\quad
	\begin{subfigure}[t]{0.35\columnwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{figures/synthetic/aperture_29_invertible.png}
		\caption*{}
		\includegraphics[width=\textwidth]{figures/synthetic/synthetic_optn_29.png}
		\caption*{}
		\includegraphics[height=1in]{figures/synthetic/synthetic_spec_29_invertible.pdf}
		\caption{Optimally invertible aperture code}
	\end{subfigure}
	\quad
	\begin{subfigure}[t]{0.35\columnwidth}
		\centering
		\includegraphics[width=0.5\textwidth]{figures/synthetic/aperture_31_imperceptible.png}
		\caption*{}
		\includegraphics[width=\textwidth]{figures/synthetic/synthetic_optm_31.png}
		\caption*{}
		\includegraphics[height=1in]{figures/synthetic/synthetic_spec_31_imperceptible.pdf}
		\caption{Optimally invertible aperture code}
	\end{subfigure}
	\caption{Effect of aperture on spatial and spectral resolution. While a slit enables high spectral resolution, spatial reoslution takes a hit. On the other hand, an open aperture enables high spatial resolution but blurs the spectrum. Optimal coded apertures enable both high spatial and spectral resolution.}
\end{figure*}
%
There are several designs for hyperspectral imaging including spatial sweep, spectral sweep, single-snapshot design and various compressive sensing (CS) solutions. 
%
One particular design is the Agile spectral camera, which uses a diffraction grating to split aperture into various wavelengths -- called a rainbow plane; by scanning this rainbow plane, we can then measure the complete hyperspectral cube.

Unfortunately, no previous work studied the effect of diffraction due to aperture coding on sharpness of image.
%
This is of paramount importance if high resolution hyperspectral images are required. 
%
Indeed, the naive design either blurs spectral measurements and has high light throughput, or blurs images and has extrememly low light throughput.
%
Fig. \ref{fig:aperture_compare} shows a comparison of various apertures and its effect on spatial and spectral blur.
%
While a slit is ideal for high spectral resolution, the spatial resolution is very poor. 
%
Similarly, an open aperture is ideal for high spatial resolution but the spectral resolution is poor. 
%
This almost seems to present a spatio-spectral uncertainty principle, which is not desirable.

The answer to this uncertainty, however, is a fairly simple solution and it goes back to the idea of artificially introducing a blur which can be inverted in post-capture phase.
%
This falls under the broad category of coded aperture imaging and has been explored in various works.
%
The idea is to move away from simple apertures like slits or fully open apertures and instead place a binary mask such that the blur introduced by the aperture can then be inverted with no loss of information.
%
This will enable high spatial resolution and simultaneously high spectral resolution.
%
An added advantage of using a coded aperture is that the light throughput is significantly increased compared to a slit -- a practical consideration since real-world systems are very noisy.
%
Over the course of this article, we will closely analyze a simple $4f$ system which will provide theoretical understanding of what happens when we place a mask at the aperture plane.
%
We then introduce coded aperture design with some broad design ideas in terms of noise performance and spatio-spectral resolution.
%
%\begin{figure}[!ttt]
%	\centering
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\includegraphics[width=0.3\textwidth]{figures/slit.png}
%		\quad
%		\includegraphics[width=0.3\textwidth]{figures/slit_space.png}
%		\quad
%		\includegraphics[width=0.3\textwidth]{figures/slit_spectrum.pdf}
%		\caption{Image and spectrum with a slit for aperture.}
%	\end{subfigure}
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\includegraphics[width=0.3\textwidth]{figures/open_9.png}
%		\quad
%		\includegraphics[width=0.3\textwidth]{figures/open_9_space.png}
%		\quad
%		\includegraphics[width=0.3\textwidth]{figures/open_9_spectrum.pdf}
%		\caption{Image and spectrum with a small aperture.}
%	\end{subfigure}
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\includegraphics[width=0.3\textwidth]{figures/open_29.png}
%		\quad
%		\includegraphics[width=0.3\textwidth]{figures/open_29_space.png}
%		\quad
%		\includegraphics[width=0.3\textwidth]{figures/open_29_spectrum.pdf}
%		\caption{Image and spectrum with a large aperture.}
%	\end{subfigure}
%	\caption{Effect of aperture on spatial and spectral resolution. A slit allows high spectral resolution but very poor spatial resolution. A large aperture on the other hand allows high spatial resolution but poor spectral resolution.}
%	\label{fig:aperture_compare}
%\end{figure}
\subsection{The $4f$ system}
\input{oc_model.tex}

\subsection{Optimal aperture codes}
\input{oc_code_design.tex}

\input{oc_synthetic.tex}

==> spacespectrum.tex <==
In this section, we introduce an optical system capable of simultaneously resolving space and spectrum at high resolutions. 
%
Along the way, we explain why traditional systems for measuring images and spectrum are mutually incompatible.
%
%The optical system described in this section provides the bed-rock for the KRISM architecture for optical computing of hyperspectral images in Section \ref{section:optical}.




%\subsection{4F systems and their properties}
%Our proposed optical setup relies extensively on 4f systems and their properties. 
%%
%In particular, we rely on properties of the two 4F systems shown in Figure \ref{fig:basic4F}.
%%
%All of these discussions assumes that the light incident  to be incoherent and hence, all effects are directly measured on the field intensity (as opposed to the complex phasor).
%
%\begin{figure}[!hhh]
%\center
%\includegraphics[width=0.475\textwidth]{figures/spacespectrum/Basic4Fs.pdf}
%\caption{Here}
%\label{fig:basic4F}
%\end{figure}
%
%\paragraph{Figure \ref{fig:basic4F}(a) --- Pupil plane coding.} Consider a 4F system with an (coded) aperture on the pupil plane; we assume the lenses to be ideal thin lenses of focal length $f$.
%%
%Since we have assumed that the incident light to be incoherent, the intensity observed at image plane P3 is simply a spatial convolution of the intensity field at the image plane P1 and the power spectral density of the coded aperture.
%%
%Specifically, if $a(x, y, \lambda)$ is the intensity field at P1, $c(x'', y'', \lambda)$ is the intensity field at P3, and $t(x', y')$ is the aperture code in the pupil plane P2,  then
%\[ c(x'', y'', \lambda) =   a(-x'', -y'', \lambda) \ast \left| T\left(\frac{x''}{\lambda f}, \frac{y''}{\lambda f} \right) \right|^2, \]
%where $\ast$ refers to 2D convolution and  $T(u, v)$ is the 2D Fourier transform of the coded aperture $t(x'', y'')$.
%%
%Equivalently, in the Fourier domain, this can be written as
%
%This is a standard result from Fourier optics and we defer the derivation to canon material \cite{}.
%
%\paragraph{Figure \ref{fig:basic4F}(b) --- Spatial  coding with a diffraction grating.} The second 4F system we consider has a diffraction grating on the image plane $P1$.
%%
%The effect of the grating can be modeled as one of multiplication the spatial intensity field $d_0(x, y, \lambda)$ with a Dirac delta train whose periodicity is giving by the grating's groove density, i.e.,
%\[ d_1(x, y, \lambda) =  d_0(x, y, \lambda) \sum_k \delta(x - k/v_0), \]
%where $v_0$ is the groove density in grooves per unit-length, and $d_1$ is the spatial intensity field after the effect of the grating.
%%
%Via the Fourier transforming property of the lens for incoherent light, we observe that the intensity field $e(x', y', \lambda)$ at the pupil plane P2 can be written as 
%%
%\begin{align*}
%e(x', y', \lambda) &= D_1\left(\frac{x'}{\lambda f}, \frac{y'}{\lambda f}, \lambda \right) \\
%&= D_0\left(\frac{x'}{\lambda f}, \frac{y'}{\lambda f}, \lambda \right) \ast \sum_m \delta \left( \frac{x'}{\lambda f} - mv_0 \right)\\
%& \propto D_0\left(\frac{x'}{\lambda f}, \frac{y'}{\lambda f}, \lambda \right) \ast \sum_m \delta \left({x'} - mv_0 {\lambda f} \right)
%\end{align*}
%In practice, gratings are optimized to be not an ideal delta train but to have a dominant mode.
%%
%Assuming that this mode corresponds to $m = 1$ in the expression above, we get
%\[ e(x', y', \lambda)  \propto D_0\left(\frac{x'}{\lambda f} - mv_0, \frac{y'}{\lambda f}, \lambda \right).  \]

\subsection{Optical setup}
\error{Shorten this section with only key results. Perhaps we can add a table with spatial and spectral blur for slit, open aperture and coded aperture.}
The optical schematic in Figure \ref{fig:schematic} has an objective lens that focus a scene onto its image plane, denoted as P1. 
%
This is followed by two 4$f$ relays with a coded aperture placed on the first pupil plane, P2, and a diffraction grating placed at the plane marked as P3.
%
We are interested in the intensity images formed at the planes marked at P4 and P5, and their relationship to the image formed on the image plane P1, the coded aperture, and the grating parameters.


We begin by assuming that the field formed on plane P1 is \textit{incoherent}; an immediate consequence of the incoherent field assumption is that we only need to consider its magnitude and how it propagates, and largely ignore its phase.
%
Let $I_1(x_1, y_1, \lambda)$ be the intensity of the field as a function of spatial coordinates $(x_1, y_1)$ and wavelength $\lambda$.
%
The Fourier transforming property of the first relay lens, coupled with the incoherence of the light, implies that we will observe a field at the first pupil plane P2 whose magnitude is largely constant; the geometric optics interpretation of this is that under Lambertian assumption, a fully defocused image of the scene has a constant intensity field.
%
This implies that the intensity field $I_2(x_2, y_2, \lambda)$, \textit{before} the coded aperture can be written as
\begin{equation}
I_2(x_2, y_2, \lambda) \propto s(\lambda),
\end{equation}
where $s(\lambda)$ is the scene's overall spectral content defined as
\begin{equation}
s(\lambda) = \int_x \int_y I_1(x, y, \lambda) dx dy.
\end{equation}
%
The coded aperture acts as an amplitude mask and its transmission is given as $a(x_2, y_2)$; hence, the 
intensity field at the plane P2 immediately after the coded aperture is simply
\begin{equation}
\widetilde{I}_2(x_2, y_2, \lambda) \propto a_2(x_2, y_2)\ s(\lambda).
\end{equation}

\begin{figure*}[!ttt]
\includegraphics[width=\textwidth]{figures/spacespectrum/Apertures_v2.pdf}
\caption{To verify the effect of different kinds of pupil codes, we implemented the setup shown in Figure \ref{fig:schematic}. An open aperture leads to sharp spatial images, but the spectrum is blurred, as is evident from the spectrum of LED + 532nm laser. On the other hand, a slit offers high spectral resolution, but the spatial image is blurred. Optimal invertible codes offer invertible spectral blur, and at the same time, invertible spatial blur.}
\label{fig:apertures}
\end{figure*}



The intensity field $I_3(x_3, y_3, \lambda)$ at the image plane P3, before the diffraction grating, is given as 
\begin{equation}
I_3(x_3, y_3, \lambda) = I_1(-x_3, -y_3, \lambda) \ast \left| A\left(\frac{x_3}{\lambda f}, \frac{y_3}{\lambda f} \right) \right|^2,
\end{equation}
where $\ast$ denotes the 2D convolution operator and $A(u, v)$ is the 2D Fourier transform of the aperture code $a(x, y)$.
%
This is a standard result from Fourier optics (see  \cite{goodman2005introduction}).

We now derive expressions for the intensity field at the rainbow plane P4 and the spatial plane P5.
%
Consider the 4$f$ system formed between P2 and P4; this system has a grating in its pupil plane P3 with a groove density of $v_0$ grooves per mm.
%
We model the diffraction grating as one that implements a spectrally-dependent phase shift; since a phase shift in the Fourier domain is equivalent to a translation in the dual, we will observe in P4  a spectrally-dependent translation of the intensity field.
%
Specifically, we can write the intensity field at the rainbow plane P4 as 
\begin{align}
I_4(x_4, y_4, \lambda) &= \widetilde{I}_2(-x_4+f\lambda v_0, -y_4, \lambda) \nonumber \\
&\propto a_2(-x_4+ f \lambda v_0, -y_4) s(\lambda)
\end{align}
%

To get the intensity field at the spatial plane P5, we can simply observe that it is 4$f$ away from the plane P3.
%
Further, a grating of sufficiently high density will not be visible to a camera placed at P5 and hence, we can write the expression for the intensity field at the spatial plane P5 as 
\begin{align}
I_5(x_5, y_5, \lambda) &= I_3(-x_5, -y_5, \lambda) \nonumber \\
&= I_1(x_5, y_5, \lambda) \ast \left| A\left(-\frac{x_5}{\lambda f}, -\frac{y_5}{\lambda f} \right) \right|^2
\end{align}




\paragraph{Image at the rainbow plane.} A camera with spectral response $c(\lambda)$ placed at the rainbow plane would measure 
\begin{align} 
I_R(x, y) &\propto \int_\lambda  a_2(-x+ f \lambda v_0, -y) s(\lambda) c(\lambda) d\lambda \nonumber\\
&\propto a_2(x, y) \ast \left(s\left(\frac{x}{f v_0}\right) c\left(\frac{x}{fv_0}\right) \right). 
\end{align}
Here, the dimensionless term $fv_0$ provides a scaling of the spectrum of the scene and indicates the resolving power of the diffraction grating.
%
For example, we use a focal length $f = 100mm$ and a grating with groove density $v_0 = 300$ grooves/mm for the prototype discussed in Section \ref{section:optical}; here,  $f v_0 = 30,000$. This implies that the spectrum is stretched by a factor of $30,000$. 
%
Therefore, a 1nm of the spectrum maps to 30 $\mu$m, which is about 6-7 pixel-widths on the cameras that we use.
%
The key insight  this expression provides is that the  image $I_R$ is the convolution of the scene's spectrum --- denoted as a 1D image --- with the aperture code $a(\cdot, \cdot)$.
%
This implies that we can measure the spectrum of the scene, albeit convolved with the aperture code on this plane; this motivates our naming of this plane as the rainbow plane.

\paragraph{Image at the spatial plane.} A camera with the spectral response $c(\lambda)$ placed at the spatial plane P5 would measure
\begin{align} 
I_S(x, y) \propto \int_\lambda \left( I_1(x, y, \lambda) \ast  \left| A\left(-\frac{x}{\lambda f}, -\frac{y}{\lambda f} \right) \right|^2 \right) c(\lambda) d\lambda
\end{align}
%
This indicates that we can measure an image of the hyperspectral intensity field at the spatial plane P5.
%
However, there is a spectrally dependent blur whose kernel is given as the power spectral density (PSD) of the aperture code, scaled by $\lambda f$.


\paragraph{Remark.} The derivation above indicates that we can measure the  spectral profile of the scene at the rainbow plane and a spatial image of the scene at the spatial plane. 
%
This, however, should not be surprising.
%
Ours is a general schematic that subsumes designs for spectrometer (via the use of grating) as well as an conventional camera.
%
A conventional spectrometer uses the exact same architecture as shown in the optical schematic ---  truncated at the rainbow plane and with a slit aperture at P2.
%
Similarly, a conventional camera would simply acquire an image of the scene by placing the sensor at P1; when an open aperture is placed at P2,  this image would be  identical to the spatial intensity at P5.
%
However, the differences in the nature of the apertures --- a slit for the spectrometer and an open aperture for an imager --- are significant in that the use of either of them leads to severe loss in our ability to resolve both space and spectrum simultaneously.




\subsection{Failure of slits and open apertures}
We now consider the effect of the traditional apertures used in imaging and spectrometry ---  namely, an open aperture and a slit, respectively --- on the images formed at the rainbow and the spatial planes.
%
Suppose that the aperture code $a(x, y)$ is a box function of width $W$ mm and height $H$ mm, i.e.,
\[ a(x, y) = \textrm{rect}_W(x)\, \textrm{rect}_H(y).\]
%
Its Fourier transform $A(u, v)$ is the product of two sincs
\[ A(u, v) = \textrm{sinc}(Wu)\, \textrm{sinc}(Hv). \]
%
Hence, the PSF has a central lobe of size $(1/W) \times (1/H)$ 1/mm$^2$.
%
The spatial image $I_S$ is convolved with the PSD $|A(u, v)|^2$ scaled by $f\lambda$ and so, the blur observed on it has a spatial extent of $f\lambda/W \times f\lambda/H$ units.
%
Suppose that $f = 100mm$ and $\lambda = 0.5 \mu$m, the observed blur is $50/W \mu$m $\times 50/H \mu$m. 
%
The rainbow plane image $I_R$, on the other hand, simply observes a box blur whose spatial extent is $W \textrm{mm} \times H$ mm.
%
Armed with these expressions, we can study the effect of an open and a slit apertures on the spatial and rainbow images.

\begin{figure*}[!ttt]
	\centering
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=0.48\textwidth]{figures/code_compare/invertible_32_code.pdf}
		\includegraphics[width=0.35\textwidth]{figures/code_compare/aperture_32_invertible.png}
		\caption{Optimized code and aperture for $N=32$.}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=0.45\textwidth]{figures/code_compare/inv32_spec_raw.pdf}
		\quad
		\includegraphics[width=0.45\textwidth]{figures/code_compare/inv32_raw.png}
		\caption{Raw measurements.}
	\end{subfigure}
	\begin{subfigure}[t]{0.32\textwidth}
		\centering
		\includegraphics[width=0.45\textwidth]{figures/code_compare/inv32_spec.pdf}
		\quad
		\includegraphics[width=0.45\textwidth]{figures/code_compare/inv32.png}
		\caption{Deconvolved spectrum and image respectively\\(Spectrum SNR: 21.5dB; Spatial RSNR: 25.3)}
	\end{subfigure}
	\caption{Binary code and measured image for an optimally imperceptible code of length 32. The invertible codes ensure that the spectral as well as spatial blur can be deconvolved. Raw measurements, and deconvolved spectrum and spatial measurements respectively. Spectrum was deconvolved using Wiener deconvolution, and spatial images were deconvolved using TV prior. Invertible codes offer resolution in spectrum and space.}
	\label{fig:code_compare}
\end{figure*}


\paragraph{Scenario \#1 --- An open aperture.} Suppose that $W = H = 10$ mm, then we can calculate the spatial blur to be $5 \mu$m, and hence, we can expect a very sharp spatial image of the scene.
%
The blur on the rainbow image however would be $10$ mm; for  relay lenses with focal length $f = 100$mm and grating with groove density $v_0 = 300$ grooves/mm, this would be equivalent of a spectral blur of $10,000/30 \approx 333$ nm.
%
Hence, we cannot hope to achieve high spectral resolution with an open aperture.

\paragraph{Scenario \#2 --- A slit.} A slit is commonly used in spectrometers; suppose that we use a slit of width $W = 100 \mu$m and height $H = 10$mm.
%
Then, we expect to see a spectral blur of $100/30 \approx 3.3$ nm.
%
The spatial image is blurred along the y-axis by a $5 \mu$m blur and along the x-axis by a 
$50/0.1 = 500 \mu$ m blur; effectively, with a $5 \mu$m pixel pitch, this would correspond to a 1D blur of 100 pixels.
%
In essence, the use of a slit leads to severe loss in spatial resolution.

Figure \ref{fig:apertures} shows images obtained with various aperture codes on a lab prototype of the schematic shown in Figure \ref{fig:schematic}.
%
These images captured with real hardware validate the derivations above.
%
In essence, jointly achieving high spatial and spectral resolutions is extremely hard in conventional imaging architectures due to the nature of the apertures used.
%
We next design a  class of apertures that have carefully engineered spectral and spatial blurs, which can be computationally deblurred in post-processing.



\subsection{Design of aperture codes}
We now design a space of codes that allow us to resolve both space and spectrum at high-resolutions.

\paragraph{Observation.} Recall that the rainbow plane image $I_R$ is a convolution between a 1D spectral profile $s(\cdot)$ and a 2D aperture code $a(x,y)$.
%
If we used a  aperture $a(x, y)$ that is separable in $x$ and $y$, then a natural choice is to use \[ a(x, y) = a(x) \textrm{rect}_H(y), \] with $H$ being as large as possible. 
%
This has two implications.
%
First, from separability of Fourier transformations as well as convolutions, we can show that the resulting spatial blur along $y$ direction is extremely small.
%
Second, for any given 1D aperture code $a(x)$, this results in the largest possible light throughput.
%
It is also worth noting that the spectral blur and its invertibility is unaffected by this choice.
%

Since binary amplitude masks are easy to fabricate, we design binary aperture codes of fixed lengths.
%
That is, we design the 1D code $a(x)$ as follows:
\begin{align}
	a(x) &= \sum\limits_{k=0}^{N-1} a_k\, \mathbb{I}_{[k \Delta, (k+1) \Delta]}(x),
\end{align}
where $\mathbb{I}_{[k\Delta, (k+1)\Delta]}(x) = 1$ when  $x \in [k\Delta, (k+1)\Delta]$ and zero otherwise.
%
Hence, the mask design reduces to finding an $N$-bit codeword ${\bf a} = \{a_1, a_2, \ldots, a_N\}$.
%
The term $\Delta$, with units in lengths, specifies the physical dimension of each bit in the code.
%
We fix its value based on the desired spectral resolution.
%
For example, for $f = 100$mm and $v_0 = 300$ grooves/mm, a desired spectral resolution of $1$nm would require $\Delta \le 30 \mu$m.

Our goal is to design masks that enable the following:
\begin{itemize}[leftmargin=*]
\item \textit{High light throughput.} For a given code length $N$, we seek codes with large light throughput which is equal to the number of ones in the code word ${\bf a}.$
\item \textit{Invertibility of the spectral blur.} The code is designed such that the resulting spectral blur is invertible.
\item \textit{Invertible spatial blur.} The code is designed such that the resulting spatial blur is invertible too.
\end{itemize}

We achieve an invertible spectral blur by ensuring that the spectrum of $a(x)$ be as flat as possible.
%
Given that the spectrum is linearly convolved with $a(x)$, a $(N + N_\lambda -1 )$-point DFT of the code word ${\bf a}$ captures all the relevant components of the PSD of $a(x)$.
%
Denoting this $(N + N_\lambda -1)$-point DFT of ${\bf a}$ as ${\bf A}[k]$, we aim to maximize its minimum value in magnitude.
%
To get invertible spatial blur, recollect that the spatial PSF is the power spectral density (PSD) of $a(x)$.
%
Hence, an invertible spatial PSF implies maximizing the minimum values of $c(x)$, the linear autocorrelation of $a(x)$. From eq. 13, we get, $c(x) = \sum\limits_{k=-N}^{N-1}c_k T_{[(k-1)\Delta, (k+1)\Delta]}(x)$, where $c_k = \sum\limits_{p=-N}^{N-1}a_p a_{p+k}$ and $T_{[(k-1)\Delta, (k+1)\Delta]}(x) = ?$.
%
Thus, it is sufficient to maximize the minimum values of $c_k$, which is easy to compute. 
%
Combining everything, the optimization function we seek is:
\begin{equation}
\max_{a_1, \ldots, a_N} \alpha \min_k \left(| {\bf A}[k] |\right) + (1-\alpha )  \min_k c_k, \quad \text{s.t.}\quad  \forall j, a_j \in \{0, 1\}
\label{eq:obj_invertible}
\end{equation}
 %
%Next, to achieve an invertible spatial blur, we maximize the minimum value of the spatial blur point spread function (PSF).
%
%Let $P_a(x)$ be the spatial PSF created by $a(x)$. If $\eta_1, \eta_2$ be the first and second maximum peak heights of $P_a(x)$, then maximizing the ratio $\eta_2/\eta_1$ leads to spatially imperceptible blur.
%
%Together, we formulate the overall objective function as:
%
%\begin{equation}
%\max_{a_1, \ldots, a_N} \alpha \min_k \left(| {\bf A}[k] |\right) + (1-\alpha )  %\left(\frac{\eta_2}{\eta_1}\right), \quad \text{s.t.}\quad  \forall j, a_j \in \{0, 1\}
%\label{eq:obj_imperceptible}
%\end{equation}
where $\alpha \in (0, 1)$ is a constant.
%
For code length $N$ sufficiently small, we can simply solve for the optimal code via exhaustive search of all $2^N-1$ code words. 
%
It is worth noting here that the our use of coded apertures is inspired by seminal works in coded photography for motion and defocus deblurring \cite{raskar2006coded,veeraraghavan2007dappled,levin2007image}.
%
%This strategy is surprisingly not time-consuming even for $N = 31$.
\subsection{Coded aperture and the scene's HSI}
The addition of the coded aperture intentionally blurs the HSI along space and spectrum.
%
Let $A$ be the linear convolution matrix that blurs the spatial images and $B$ be the linear convolution matrix that blurs the spectral profiles. 
%
Then the effective HSI is $\widetilde{X} = AXB$. 
%
When the HSI $X$ is low-rank,  the blurred HSI $\widetilde{X}$ is also low-rank.
%
We can effectively apply Krylov subspace techniques to the blurred HSI and subsequently, deblur the capture singular vectors to obtain the low-rank approximation to $X$.
%
All our real experiments were performed keeping this model in mind, where we deconvolved the spatial and spectral singular vectors, in post capture.

\begin{comment}
\subsection{Performance analysis}
\note{Might want to completely move this to supplementary, and just add some notes about MTF and obtained spectral resolution}
Figure \ref{fig:code_compare} shows the aperture code for $N=31$ and a simulation result on a hyperspectral scene with spatial texture of a resolution chart and spectrum given by two closely spaced peaks.
%
Note that the spatial blur with the imperceptible code is barely visible, which makes it an optimal choice for high-resolution image measurements.
%
The measurements were simulated with 30dB noise level. 
%
We used deconvolution with a Total Variance (TV) prior for images \cite{bioucas2007new} and Richardson Lucy for spectrum.
%
\paragraph{Spatial and spectral resolutions with imperceptible codes.} We evaluated spatial resolution using MTF30 on the lab prototype described in Section \ref{section:optical}. MTF30 is defined as the number of line pairs per pixel which have contrast ratio grater than 30\%. 
%
MTF30 was computed by focusing on a Siemens star resolution chart placed in front of the camera.
%
We then compute the contrast ratio for four sectors at each radius, which gives us a plot of contrast ratio as a function of line pairs per pixel. 
%
To enhance the results, we deconvolved the image of Siemens star by the PSF of the imperceptible code.
%
The PSF was obtained by placing a $10\mu m$ pinhole in front of the camera and recording its image.
%
The image of the pinhole was then used as an initial guess for blind deconvolution.
%
Figure \ref{fig:space_res} shows the image of the Siemens star captured by our setup, the deconvolved image using the estimate PSF, as well as the MTF30 plots on two sectors of the image.
%Figure \ref{fig:space_res} (\textbf{a}) shows the image of Siemens star captured by our setup with sectors clearly marked.
%%
%Figure \ref{fig:space_res} (\textbf{b}) shows the image of Siemens star after deconvolution using the estimated PSF.
%%
%Figure \ref{fig:space_res} (\textbf{c}) shows results for MTF computation for spatial measurements. Prior to deconvolution, MTF30 value for horizontal sector is 0.15 lp/pixels, whereas that for vertical direction is 0.2 lp/pixel. 
%
After deconvolution, MTF30 is 0.3 lp/pixels for horizontal direction and greater than 0.5 lp/pixels for vertical direction.
%
Having a compact spatial blur implies that the spatial resolution is good even prior to deconvolution.
%
%Added to this, deconvolution is easier with a compact spatial blur.

Spectral resolution was evaluated by placing several narrow band filters in front of a  bright light source.
%
Figure \ref{fig:spectrum_res} shows the spectra of various narrowband filters. 
%The estimated central wavelengths and FWHM from our optical system (in nm) was 438.8 (10.5), 456.4 (27.7), 488.1 (2.9), 514.4 (2.9), 583.6 (7.6), 669.9 (3.8), 640.2 (41.5), and 731.1 (11.1)  respectively.
%
Measured spectra was then deconvolved using Richardson-Lucy iterative method to obtain true spectra of the filters.
%
Assuming each filter to have a Gaussian distribution and that our optical system has a Gaussian distribution too, the FWHM of our system is $\sqrt{2.92^2-1^1} = 2.7 nm$.
%
\begin{figure}[!ttt]
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/mtf/imstar.png}
	\end{subfigure}
	\quad
	\setcounter{subfigure}{2}
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/mtf/mtf.pdf}
		\caption{MTF for various sectors before and after deconvolution.}
	\end{subfigure}
	\caption{Evaluation of spatial resolution. We placed a Siemen star in front of our camera (\textbf{a}) and evaluate the MTF (\textbf{a}) over two sectors. The resolution target was then deconvolved with a PSF we estimated by placing a pinhole in front of our camera to obtain (\textbf{b}), which gives a sharper spatial image. The MTF before and after deconvolution is shown in (\textbf{c}). There is a doubling of Nyquist frequencies in both sectors after deconvolution.}
	\label{fig:space_res}
\end{figure}
\begin{figure}[!ttt]
	\centering
	\includegraphics[width=\columnwidth]{figures/real_imperceptible/filters.pdf}
	\caption{To evaluate spectral resolution, we used a broadband light and several narrowband filters in succession. Spectra of the filters were then obtained by deconvolving the measurements using Richardson-Lucy method. The ground truth central wavelength and its FWHM are shown in the legend. The estimated central wavelengths (and their FWHM) from our optical system were 438.8 (10.5), 456.4 (27.7), 488.1 (2.9), 514.4 (2.9), 583.6 (7.6), 669.9 (3.8), 640.2 (41.5), and 731.1 (11.1)  respectively, in nm. From this, we compute the FWHM of our system to be approximately 2.7nm.}
	\label{fig:spectrum_res}
\end{figure}
%
\end{comment}

==> sup_conclusion.tex <==
We presented a novel optical computing technique called KRISM in the main paper, and showed several compelling simulations and measurements with our lab prototype.
%
The supplementary material showed several more simulation results, establishing the effectiveness of KRISM across a diverse set of datasets.
%
We added detailed information about the optical setup we built, with emphasis on design choices.
%
We believe that this will enable democratization of the optical setup, and would engender further research in adaptive sensing of similar low-rank volumes.

\paragraph{Video rate camera.} Since KRISM captures HSI with only a few measurements, with no post processing, video-rate imagery is imminent. However, we faced several challenges with our lab prototype. We list them here, with solutions on how to overcome them.
%
\begin{enumerate}[leftmargin=*]
	\item \textit{Low $F/\#$}: Recollect that our optical setup exhibits $F/\# = F/22$, which significantly hampers its light collection abilities. This increases the exposure time per capture. This is mainly due to the 100mm lenses used in the optical setup, which was chosen due to mechanical restrictions of off-the-shelf components. Significant improvements are possible even with 50mm lenses, which increase light collection to $F/11$.
	%
	\item \textit{Camera sensitivity}: We use machine vision camera (Pointgrey Blackfly) with a dynamic range of 72dB and peak quantum efficiency of 80\%, which is significantly low compared to scientific cameras. This requires multiple averages to reduce the noise in the system. Switching to scientific cameras would further reduce the capture time.
	%
	\item \textit{Slow LCoS}: We currently use a Holoeye HES 6001 LCoS which is controlled via HDMI cable, restricting the video rate to 60fps. Further, the setup was controlled from Matlab code, adding further overhead. Switching to a dedicated hardware controller, such as an FPGA would drastically reduce the latency.
	%
	\item \textit{LC rotator}: Last but not the least, we used off-the-shelf LC rotators which had a settling time of 100ms. Switching to Ferroelectric shutters will bring down the latency to 1ms, thus reducing the overall latency.
\end{enumerate}
%
With the suggested modifications, we easily envision a high spatio-spectral resolution and video rate Hyperspectral camera.
%


==> theory.tex <==
% Theory file about noise and minimum number of measurements

We outline proofs for recovery accuracy of our method and number of measurements for good representation.

\subsection{Number of measurements}
We compare the least number of measurements for our proposed method against Nyquist sensing techniques and row and column projection based CS recovery \cite{fazel2008compressed}. 
%
We assume recovery of a rank $k$ hyperspectral image of $N_1 \times N_2$ spatial dimension and $N_3$ spectral bands. 
%

\paragraph{Full hyperspectral image sensing.}
Techniques such as tunable filter based sensing or pushbroom sensing work by sensing every element of the hyperspectral cube. 
%
Under such conditions, it is clear that the number of measurements is,
\begin{align}
	M_\textrm{Nyquist} = N_1 N_2 N_3
\end{align}

\paragraph{CS technique.} Chen et al. \cite{chen2011robust} showed that for a matrix of size $m\times n$ which can be expressed as a sum of a rank-$k$ matrix and sparse non-zero columns, robust recovery is guaranteed with high probability under the following conditions,
\begin{align}
p &\gtrsim \frac{k\log^2(m+n)}{\min(m,n)}\\\nonumber
\gamma &\lesssim \frac{p}{k\sqrt{k}\log^3(m+n)},\nonumber
\end{align}
where $p$ is the fraction of observations and $\gamma$ is the fraction of non-zero columns in the sparse matrix. Adapting it to our method, we have
\begin{align}
\label{eq:m_joint}
M_{\text{joint}} &\gtrsim \frac{N_1 N_2 N_3 k\log^2(N_1 N_2 + N_3)}{\min(N_1 N_2 , N_3)}\\ \nonumber
&= kN_1 N_2 \log^2(N_1 N_2 + N_3), \nonumber
\end{align}
where $M_\text{joint}$ is the number of measurements for joint recovery of sparse and low rank matrices. 

\paragraph{Proposed method.}
Our method relies on the power method, which computes eigenvectors through a series of matrix vector multiplies, which, adopted to our scenario is a series of spatial and spectral measurements.
%
Assume that a rank $k$ estimate of a matrix requires $ak+b$ power iterations, where $a, b$ are constants. 
%
For our power method, we require $N_1 N_2$ measurements for every spatial measurement and $N_3$ for every spectral measurement.
%
Under such conditions, the number of measurements required,
\begin{align}
	M_\textrm{power} &= (ak+b)(N_1 N_2 + N_3).
\end{align}
%
It is clear that our proposed method requires the least number of measurements of the three methods compared above. 

\subsection{Accuracy of recovery}
For a fair comparison, we contrast accuracy of rank $k$ estimate of a noisy measurement of the complete cube, CS based recovery with noisey measurements and our proposed method, which directly estimates a rank $k$ hyperspectral image.

We assume that each measurement is corrupted by additive white gaussian noise (AWGN). Hence, any measurement can be written as, $y = x + n$, where $n \sim \mathcal{N}(0, \sigma^2)$.
%
\paragraph{Full hyperspectral image sensing.}
In case of complete hyperspectral imaging, measurement noise is the only source of noise. Hence, the error of measurement,
%
\begin{align}
	\|X - X_\textrm{Nyquist}\|^2_F = N_1 N_2 N_3 \sigma^2. 
\end{align}

Let $\sigma_1 > \sigma_2 > \cdots > \sigma_{N_3}$ be the non-zero singular values of $X$. Since we are looking at a rank-6 approximation, we have,
\begin{align}
	\| X_\textrm{Nyquist} - X \|_F &= \| X_\textrm{Nyquist} - Y + Y - X \|_F \nonumber \\
						  &\le \|X_\textrm{Nyquist} -Y \|_F + \|Y - X\|_F\nonumber \\
						  &= \sqrt{\sum_{i=k}^{N_3}\sigma^2_i} + \sqrt{N_1 N_2 N_3 \sigma^2}
\end{align}

\paragraph{CS techniques.}
We will be looking at low rank + sparse recovery of a matrix from its compressive measurements. The results are based on Robust PCA with compressive measurements by \cite{ha2015robust}. The measurement model is assumed to be,
\begin{align}
	Y = (L^* + S^*).C + Z,
	\label{eq:cvx_modl}
\end{align}
where $L^* \in \rdim{N_1 N_2 \times N_3}$ is the low rank component, $S^* \in \rdim{N_1 N_2 \times N_3}$ is the row sparse component, $C \in \rdim{M \times N_3}$ is the compression matrix and $Z$ is added noise such thatn $Z_{i, i} \sim \mathcal{N}(0, \sigma^2)$. Let $P = LC$. The components are recovered as a solution to the following convex program,
\begin{align}
	(\hat{P}, \hat{S}) = \nonumber\\ \arg \min_{(P,S):\|PC^\top\|_\infty \alpha} \left\{ \frac{1}{2}\|Y-P-S.C\|^2_2 + \nu \|P\|_* + \lambda \|S\|_{2,1} \right\}.
	\label{eq:cvx_program}
\end{align}
Under such model and solution and assuming $C$ to be random sub-gaussian, we have the following guarantees.

\begin{theorem1} \textit{Adapted from Theorem 2 in \cite{ha2015robust}}
	
	Let rank $(L^*) \le k$, $\max_i \|S^*_{i*}\| \le s$ and $\|L^*\|_\infty \le \alpha_0$. Then there exist universal constants $c, c^\prime, c^{\prime\prime}>0$ such that, if we define,
	\begin{align*}
		\alpha = 5\alpha_0 \sqrt{\frac{M\log(N_1 N_2 M)}{N_3}}, \nu = 24\sigma \sqrt{\frac{M(N_1 N_2 + N_3)}{N_3}}, \\
		\lambda = 32 \sigma \sqrt{\frac{M\log(N_1 N_2 M)}{N_3}} + 4\alpha,
	\end{align*}
	and $N_3 \ge cs\log(N_1 N_2 M)$, then the solution $(\hat{P}, \hat{S})$ to the convex program \ref{eq:cvx_program} satisfies
	\begin{align}
		\|\hat{P} - P^*\|^2_F + \| \hat{S} - S^* \|^2_F \le \nonumber\\
		c^\prime \frac{M}{N_3}(\sigma^2 k (N_1 N_2 + N_3) + (\sigma^2 + \alpha_0^2)sN_1 N_2 \log(N_1N_2 M)),
	\end{align} 
	with probability at least $1 - \frac{c^{\prime \prime}}{N_1 N_2 M}$
\end{theorem1}

\paragraph{Proposed method.}
Although we use the Arnoldi method for all our computations, we use results from the subspace method, which is similar in spirit. We adopt results from \cite{hardt2014noisy} which shows accuracy of the power method under noisy settings. While results shown are for a symmetric matrix, they can be easily extended to asymmetric matrices. In particular, we adopt Corollary 1.1 to our setting.


\begin{theorem1} \textit{Adapted from Corrollary 1.1 in \cite{hardt2014noisy}}	
	Let $k\le p$. Let $U \in \rdim{N_3 \times k}$ represent the top $k$ singular vectors of $X$ and let $\sigma_1 \ge \cdots \sigma_n \ge 0$ denote its singular values. Suppose $X_0$ is an orthonormal basis of a random $p$-dimensional subspace. Further, suppose that at every step of the power method, we have,
	\begin{align*}
		5\| G_l \| &\le \epsilon(\sigma_k - \sigma_{k+1}) \quad \textrm{and} \\ 5\| U^\top G_l \| &\le (\sigma_k - \sigma_{k+1}) \frac{\sqrt{p} - \sqrt{k-1}}{\tau \sqrt{d}}
	\end{align*}
	for some fixed parameter $\tau$ and $\epsilon \le 1/2$. Then with all but $\tau^{-\Omega(p+1-k)}+e^{-\Omega(d)}$ probability, there exists an $L=\mathcal{O}\left( \frac{\sigma_k}{\sigma_k - \sigma_{k+1}} \log(d\tau/\epsilon)\right)$ so that after L steps we have 
	\begin{align*}
		\| (I - X_L X^\top_L)U\|\le \epsilon
	\end{align*}
\end{theorem1}

The above theorem states that with sufficient number of iterations, we can be arbitrarily close to the true subspace, and that this scaling depends on the gap between subsequent eigen values. In practice, hyperspectral images have very large gap for the first few eigenvalues which helps in quick convergence of the power method.

==> tog_changes.tex <==
% List out all changes here
\subsection{Main paper}
\begin{enumerate}
	\item \textit{L274 - L280}: Added discussion about \cite{arguello2013rank,rueda2016compressive,rueda2017high}.
	
	\item \textit{Figure 2, L128 - L133}: Changed y-axis from reconstruction SNR to peak SNR (PSNR)
	
	 \item \textit{Figure 7, L799 - L829}: Changed all evaluation metrics to PSNR. Removed sentence that states that KRISM is better than Choi et al.
	 
	 \item \textit{Figure 8, L913 - L947}: Changed evaluation metrics to PSNR.
	 
	 \item \textit{Figure 13, L1255 - L1277}: Cosmetic changes to graph.
\end{enumerate}

\subsection{Supplementary document}
\begin{enumerate}
	\item \textit{Figure 3, L457 - L492}: Changed evaluation metrics to PSNR.
	
	\item \textit{Figure 13, L1027 - L1072}: Changed evaluation metrics to PSNR.
	
	\item \textit{Figure 16, L1269 - L1300}: Changed evaluation metrics to PSNR.
	
	\item \textit{Figure 17, L1369 - L1425}: Changed evaluation metrics to PSNR.
	
	\item \textit{Figure 18, 19, L1483 - L1510}: Changed evaluation metrics to PSNR.
	
	\item \textit{Figure 22, R1540 - R1583}: Changed evaluation metrics to PSNR.
	
	\item \textit{Figure 20, 21, L1597 - L1644}: Changed evaluation metrics to PSNR.
\end{enumerate}

==> xstring.tex <==
%  __________________________________________________
% |                                                  |
% |                                                  |
% |                   xstring v1.7c                  |
% |                                                  |
% |                  13 octobre 2013                 |
% |                                                  |
% |__________________________________________________|
%
% This is xtring.tex
%
% "xstring" package consists of the 7 following files:
%   xstring.tex (this file)
%   xstring.sty
%   README
%   xstring_doc_fr.tex, xstring_doc_fr.pdf (manual in french)
%   xstring_doc_en.tex, xstring_doc_en.pdf (manual in english)
%
% Christian Tellechea 2008-2013
% email : unbonpetit@gmail.com
% -------------------------------------------------------------------
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%
%     http://www.latex-project.org/lppl.txt
%
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
% -------------------------------------------------------------------
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Christian Tellechea
% -------------------------------------------------------------------
\def\xstringversion     {1.7c}
\def\xstringdate        {2013/10/13}
\def\xstringfrenchdate  {13 octobre 2013}
\def\xstringenglishdate {13 october 2013}
\edef\CurrentAtCatcode  {\the\catcode`\@}
\catcode`\@=11
\newwrite\@xs@message% canal pour les messages
\newcount\integerpart
\newcount\decimalpart% compteurs utilis\'es par xstring

\expandafter\ifx\csname @latexerr\endcsname\relax% on n'utilise pas LaTeX ?
	\immediate\write\m@ne{Package: xstring \xstringdate\space\space v\xstringversion\space\space String manipulations}%
	\long\def\@firstoftwo#1#2{#1}
	\long\def\@secondoftwo#1#2{#2}
	\long\def\@gobble#1{}
	\long\def\@ifnextchar#1#2#3{%
		\let\reserved@d=#1%
		\def\reserved@a{#2}%
		\def\reserved@b{#3}%
		\futurelet\@let@arg\@ifnch}
	\def\@ifnch{%
		\ifx\@let@arg\@sptoken
			\let\reserved@c\@xifnch
		\else
			\ifx\@let@arg\reserved@d
				\let\reserved@c\reserved@a
			\else
				\let\reserved@c\reserved@b
			\fi
		\fi
		\reserved@c}
	\def\:{\let\@sptoken= } \:
	\def\:{\@xifnch} \expandafter\def\: {\futurelet\@let@arg\@ifnch}
	\def\@ifstar#1{\@ifnextchar *{\@firstoftwo{#1}}}
	\long\def\@testopt#1#2{\@ifnextchar[{#1}{#1[{#2}]}}
	\def\@empty{}
\fi% fin des d\'efinitions LaTeX

\long\def\@xs@ifempty#1{%
	\expandafter\ifx\expandafter\relax\detokenize{#1}\relax
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}
% Ouvre un groupe o\`u les catcodes sont \`a 12 et \`a 10 pour les espaces
% ensuite, appelle \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\@xs@MakeVerb{% lit 1 argument et le transforme en verb
	\begingroup% groupe o\`u les catcodes sont \`a 12 pour la lecture suivante
		\def\do##1{\catcode`##112\relax}%
		\dospecials% on entre dans le mode verb
		\obeyspaces% et on tient compte des espaces
		\@xs@ReadVerb% et on va lire l'argument
}

% D\'efinit \@xs@ReadVerb qui lit un argument entre d\'elimiteurs verb
\def\setverbdelim#1{% d\'efinit quel est le d\'elimiteur de verb
	\expandafter\@xs@ifempty\expandafter{\@gobble#1}%
		\relax
		{\begingroup
			\newlinechar`\^^J%
			\immediate\write\@xs@message
			{Package xstring Warning: verb delimiter is not a single token on input line \the\inputlineno^^J}%
		\endgroup
		}%
	\def\@xs@ReadVerb##1#1##2#1{% lit ##2 qui est entre les d\'elimiteurs de verb
		\endgroup% on ferme le groupe
		\@xs@afterreadverb{##2}}% on appelle l'ex\'ecution de fin
}

% Assigne l'argument entre d\'elimiteur verb dans la sc #1' +
\def\verbtocs#1{%
	\def\@xs@afterreadverb##1{\def#1{##1}}%
	\@xs@MakeVerb
}

\begingroup
	\catcode\z@3 \def\@xs@twochars{^^00}%
	\catcode\z@7 \xdef\@xs@twochars{\@xs@twochars^^00}%
\endgroup

\edef\@xs@reserved@A{\long\def\noexpand\@xs@AssignResult##1\@xs@twochars}

\@xs@reserved@A#2{\endgroup\expandafter\def\expandafter#2\expandafter{\@gobble#1}}

\def\tokenize#1#2{%
	\begingroup
		\@xs@def\@xs@reserved@A{#2}% on d\'eveloppe en accord avec \fullexpandarg ou \noexpandarg
		\everyeof\expandafter{\@xs@twochars#1}% met "^^@^^@#1" \`a la fin du fichier virtuel
		\endlinechar\m@ne
		\expandafter\@xs@AssignResult\scantokens\expandafter{\expandafter\relax\@xs@reserved@A}% on fait l'assignation
}%

% Macro tr\`es simple qui assigne ou affiche le r\'esultat, selon la pr\'esence
% ou non de #2 qui est l'argument optionnel venant en derni\`ere position des macros
\long\def\@xs@ReturnResult#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#2}%
		\@xs@argument@A
		{\let#2\@xs@argument@A}%
}

\def\@xs@ldef{\long\def}

\def\@xs@ledef{\long\edef}

% Pas d'expansion des arguments
\def\normalexpandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter{##1}}}
\let\noexpandarg\normalexpandarg% synonyme

% 1-d\'eveloppement du premier token des arguments
\def\expandarg{%
	\let\@xs@def\@xs@ldef% on d\'efinit \@xs@call avec \def
	\def\@xs@expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

% D\'eveloppement maximum des arguments
\def\fullexpandarg{%
	\let\@xs@def\@xs@ledef% on d\'efinit\@xs@call avec \edef
	\def\@xs@expand##1{##1}% et on neutralise \@xs@expand
}

\def\saveexpandmode{\let\@xs@saved@def\@xs@defarg\let\@xs@saved@expand\@xs@expand}

\def\restoreexpandmode{\let\@xs@defarg\@xs@saved@def\let\@xs@expand\@xs@saved@expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\@xs@ifbeginwithbrace#1{%
	\csname @%
		\expandafter\@gobble\string{%
		\expandafter\@gobble\expandafter{\expandafter{\string#1}%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@firstoftwo
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter\@gobble
		\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\@gobble\string}%
		\@secondoftwo{first}{second}oftwo%
	\endcsname
}

% Cette macro interne prend la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@returnfirstsyntaxunit#1#2{%
	\def\@xs@groupfound{\expandafter\def\expandafter#2\expandafter{\expandafter{#2}}\@xs@gobbleall}% on met #2 dans des accolades et on finit
	\long\def\@xs@assignfirsttok##1##2\@xs@nil{\let\@xs@toks0\def#2{##1}}%
	\def\@xs@testfirsttok{%
		\let\@xs@next\@xs@assignfirsttok
		\ifx\@xs@toks\bgroup
			\expandafter\@xs@ifbeginwithbrace\expandafter{\@xs@argument}{\def\@xs@next{\afterassignment\@xs@groupfound\def#2}}{}%
		\fi
		\@xs@next}%
	\def\@xs@argument{#1}%
	\edef\@xs@next{\expandafter\@xs@beforespace\detokenize{#1} \@xs@nil}% #1 commence par un espace ?
	\ifx\@xs@next\@empty
		\def\@xs@next{\expandafter\ifx\expandafter\@empty\detokenize\expandafter{\@xs@argument}\@empty\let#2\@empty\else\def#2{ }\let\@xs@toks0\fi}%
	\else
		\def\@xs@next{\expandafter\futurelet\expandafter\@xs@toks\expandafter\@xs@testfirsttok\@xs@argument\@xs@nil}%
	\fi
	\@xs@next
}

% Cette macro interne enl\`eve la 1ere unit\'e syntaxique de #1 et assigne le r\'esultat \`a #2
\long\def\@xs@testsecondtoken#1\@xs@nil{\@xs@ifbeginwithbrace{#1}}

\long\def\@xs@gobblespacebeforebrace#1#{}% supprime tout ce qui est avant la 1ere accolade ouvrante

\long\def\@xs@removefirstsyntaxunit#1#2{%
	\def\@xs@argument{#1}%
	\expandafter\expandafter\expandafter\ifx\expandafter\expandafter\expandafter\@empty\expandafter\@xs@beforespace\detokenize\expandafter{\@xs@argument} \@xs@nil\@empty% #1 commence par un espace ?
		\expandafter\@xs@ifempty\expandafter{\@xs@argument}%
			{\let#2\@empty}
			{\afterassignment\@xs@testsecondtoken% après avoir mangé le 1er token, on va tester si la suite commence par «{»
			\expandafter\let\expandafter\@xs@secontoken\expandafter=\expandafter\@sptoken\@xs@argument\@xs@@nil\@xs@nil% on mange le 1er token et on rajoute \@xs@@nil à la fin pour éviter de perdre les accolades du groupe
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@gobblespacebeforebrace\@xs@argument}}%
				{\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
				 \expandafter\expandafter\expandafter{\expandafter\@xs@behindspace\@xs@argument\@xs@nil}}%
			}%
	\else
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter#2%
		\expandafter\expandafter\expandafter{\expandafter\@gobble\@xs@argument}%
	\fi
}

% Macros \`a arguments d\'elimit\'es pour les macros ci dessus
\long\def\@xs@beforespace#1 #2\@xs@nil{#1}

\long\def\@xs@behindspace#1 #2\@xs@nil{#2}

\long\def\@xs@returnfirstsyntaxunit@ii#1#2\@xs@nil{#1}

\long\def\@xs@gobbleall#1\@xs@nil{}

% Cette macro interne est utilis\'ee dans les macros \'etoil\'ees pour :
% 1) d\'evelopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci \`a l'aide de la macro \@xs@def
% 2) Ensuite, on d\'etokenize ce d\'eveloppement de façon n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\@xs@expand@and@detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\@xs@expand#1}% on d\'eveloppe #2 selon le mode de d\'eveloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d\'etokenize et on assigne \`a #1
}

\long\def\@xs@expand@and@assign#1#2{\@xs@def#1{#2}}% on d\'eveloppe #2 selon \fullexpandarg ou \normalexpandarg

\long\def\@xs@edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}

\long\def\@xs@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\@xs@argstring{0########1########2########3########4########5########6########7########8########9}

% \@xs@DefArg{3} met dans la sc \@xs@myarg les tokens "####1####2####3"
\def\@xs@DefArg#1{\def\@xs@defarg0##1#1##2\@xs@nil{\def\@xs@myarg{##1#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@DefArg@{3} met dans la sc \@xs@myarg les tokens "[####1]####2####3####4"
\def\@xs@DefArg@#1{\expandafter\@xs@defarg@\expandafter{\number\numexpr#1+1}}

\def\@xs@defarg@#1{\def\@xs@defarg0##11##2#1##3\@xs@nil{\def\@xs@myarg{[##11]##2#1}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% \@xs@OneArg{3} met dans la sc \@xs@myarg les tokens "####3"
\def\@xs@OneArg#1{\expandafter\@xs@onearg\expandafter{\number\numexpr#1-1}{#1}}

\def\@xs@onearg#1#2{\def\@xs@defarg##1#1##2#2##3\@xs@nil{\def\@xs@myarg{##2#2}}\expandafter\@xs@defarg\@xs@argstring\@xs@nil}

% #1 : num\'ero du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num\'ero de l'argument devant être d\'etokenis\'e si \'etoile
\def\@xs@BuildLines#1#2#3#4{%
	\let\@xs@newlines\@empty
	\let\@xs@newargs\@empty
	\def\@xs@buildlines##1{%
		\expandafter\@xs@OneArg\expandafter{\number\numexpr##1+#1-1}%
		\edef\@xs@reserved@B{\noexpand\@xs@expand\csname @xs@arg@\romannumeral\numexpr##1\endcsname}%
		\ifnum##1=\@ne% si c'est le premier argument
			\@xs@ifempty{#3}%
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
				\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
				}% et s'il y a un argument optionnel alors, on met des crochets
				{\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter[\@xs@reserved@B]}%
				\def\@xs@reserved@B{@xs@def}% ne pas d\'etok\'eniser l'argument optionnel grace au \@xs@def
				}
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@newargs\expandafter{\expandafter{\@xs@reserved@B}}%
			\edef\@xs@reserved@B{\ifnum##1>#4 @xs@def\else @xs@assign\fi}%
		\fi
		\edef\@xs@newlines{\unexpanded\expandafter{\@xs@newlines}\expandafter\noexpand\csname\@xs@reserved@B\endcsname\expandafter\noexpand\csname @xs@arg@\romannumeral\numexpr##1\endcsname{\@xs@myarg}}%
		\ifnum##1<#2\relax
			\def\@xs@next{\expandafter\@xs@buildlines\expandafter{\number\numexpr##1+1}}%
			\expandafter\@xs@next
		\fi}%
	\@xs@buildlines\@ne
}

\def\@xs@newmacro{%
	\@ifstar
		{\let\@xs@reserved@D\@empty\@xs@newmacro@}
		{\let\@xs@reserved@D\relax\@xs@newmacro@0}%
}

% #1 : dernier num\'ero de l'argument devant être d\'etokenis\'e
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\@xs@newmacro@#1#2#3#4#5{%
	\edef\@xs@reserved@A{@xs@\expandafter\@gobble\string#2}%
	\edef\@xs@reserved@C{\expandafter\noexpand\csname\@xs@reserved@A @\ifx\@empty#3\@empty @\fi\endcsname}%
	\edef\@xs@reserved@B{%
		\ifx\@empty\@xs@reserved@D
			\def\noexpand#2{\noexpand\@ifstar
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@detokenize\expandafter\noexpand\@xs@reserved@C}%
				{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\@xs@assign\noexpand\@xs@expand@and@assign\expandafter\noexpand\@xs@reserved@C}%
		\fi
		\ifx\@empty#3\@empty
		\else
			\def\expandafter\noexpand\@xs@reserved@C{%
				\noexpand\@testopt{\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname}{\ifx\@xs@def\@xs@ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit :
	% si #3 est vide : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@@}}
	% si #3 existe   : \NOM{\@ifstar{\let\@xs@assign\@xs@expand@and@detokenize\@xs@NOM@}{\let\@xs@assign\@xs@expand@and@assign\@xs@NOM@}}
	%                  \@xs@NOM@{\@testopt{\@xs@NOM@@}{#3}}}
	\long\@xs@reserved@B
	\ifx\@empty#3\@empty
		\@xs@BuildLines1{#4}{#3}{#1}%
		\@xs@DefArg{#4}%
	\else
		\expandafter\@xs@BuildLines\expandafter1\expandafter{\number\numexpr#4+1}{#3}{#1}%
		\@xs@DefArg@{#4}%
	\fi
	\edef\@xs@reserved@B{\def\expandafter\noexpand\csname\@xs@reserved@A @@\endcsname\@xs@myarg}%
	\edef\@xs@reserved@C{\unexpanded\expandafter{\@xs@newlines}\edef\noexpand\@xs@call}%
	\edef\@xs@reserved@D{%
		\noexpand\noexpand\expandafter\noexpand\csname\@xs@reserved@A\endcsname\unexpanded\expandafter{\@xs@newargs}%
	}%
	\ifnum#5=\@ne\edef\@xs@reserved@D{\noexpand\noexpand\noexpand\@testopt{\unexpanded\expandafter{\@xs@reserved@D}}{}}\fi
	\@xs@edefaddtomacro\@xs@reserved@C{{\unexpanded\expandafter{\@xs@reserved@D}}\noexpand\@xs@call}%
	\@xs@edefaddtomacro\@xs@reserved@B{{\unexpanded\expandafter{\@xs@reserved@C}}}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\@xs@NOM@@[##2]##3##4##5{%
	%          \@xs@def\@xs@arg@i{##2}\@xs@assign\@xs@arg@ii{##3}\@xs@assign\@xs@arg@iii{##4}\@xs@asign\@xs@arg@iv{##5}%
	% si #5=0: \edef\@xs@call{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}%
	% si #5=1: \edef\@xs@call{\noexpand\@testopt{\noexpand\@xs@NOM[\@xs@expand\@xs@arg@i]{\@xs@expand\@xs@arg@i}{\@xs@expand\@xs@arg@ii}{\@xs@expand\@xs@arg@iii}{\@xs@expand\@xs@arg@iv}}{}}%
	%          \@xs@call}
	\long\@xs@reserved@B
	\edef\@xs@reserved@B{%
		\def\expandafter\noexpand\csname\@xs@reserved@A\endcsname
			\@xs@myarg\ifnum#5=\@ne[\unexpanded{##}\number\numexpr\ifx\@empty#3\@empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \@xs@reserved@B ? Il d\'efinit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \@xs@NOM[##2]##3##4##5[##6]{#6}
	\long\@xs@reserved@B
}

% macro g\'en\'erique qui lit \@xs@reserved@C us par us
% 3 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atbegingroup      (un groupe vient d'être ouvert)
% \@xs@atnextsyntaxunit  (la future US n'est pas un groupe)
\def\@xs@read@reserved@C{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@read@reserved@C
		\@xs@exploregroups
		\ifx\bgroup\@xs@toks
			\advance\integerpart\@ne
			\begingroup
				\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
				\@xs@manage@groupID
				\let\@xs@nestlevel\@ne
				\integerpart\z@
				\@xs@atbegingroup
		\else
			\global\advance\decimalpart\@ne
			\@xs@atnextsyntaxunit
		\fi
		}%
	\@xs@next
}

% macro g\'en\'erique qui lit \@xs@reserved@D en proc\'edant \`a des tests avec \IfBeginWith
% 2 sous-routines sont appel\'ees \`a des moments cl\'e :
% \@xs@atendofgroup      (un groupe se finit, appel r\'ecursif)
% \@xs@atoccurfound      (une occurrence a \'et\'e trouv\'ee)
\def\@xs@read@reserved@D{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\let\@xs@next\@xs@atendofgroup
		\fi
		}%
		{\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
			{\expandafter\@xs@reserved@D\expandafter}\expandafter{\@xs@reserved@E}%
			{\global\advance\decimalpart\@ne
			\let\@xs@reserved@D\@xs@reserved@A
			\@xs@atoccurfound
			}%
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@A
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
			\let\@xs@next\@xs@read@reserved@D
			\@xs@exploregroups
			\ifx\bgroup\@xs@toks
				\advance\integerpart\@ne
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@D\@xs@reserved@A
					\@xs@manage@groupID
					\let\@xs@reserved@C\@empty
					\let\@xs@nestlevel\@ne
					\integerpart\z@
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro\StrRemoveBraces{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\let\@xs@reserved@B\@empty
	\let\@xs@nestlevel\z@
	\@xs@StrRemoveBraces@i
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#2}%
}

\def\@xs@StrRemoveBraces@i{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel=\z@
			\let\@xs@next\relax
		\else
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@B}%
			\let\@xs@next\@xs@StrRemoveBraces@i
		\fi
		}
		{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
		\let\@xs@next\@xs@StrRemoveBraces@i
		\ifx\bgroup\@xs@toks
			\ifx\@xs@exploregroups\relax% on explore les groupes ?
				\begingroup
					\expandafter\def\expandafter\@xs@reserved@C\@xs@reserved@A
					\let\@xs@nestlevel\@ne
					\integerpart\z@
					\let\@xs@reserved@B\@empty
			\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\@xs@reserved@A
			\fi
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
		\fi
		}%
	\@xs@next
}

% \@xs@cutafteroccur coupe l'argument #1 apr\`es la #3\`eme occurrence de #2
% \@xs@reserved@C : contient ce qui se trouve avant cette occurrence
% \@xs@reserved@D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \@xs@reserved@E : contient ce qui se trouve apr\`es l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy\'ees sont vides
\long\def\@xs@cutafteroccur#1#2#3{%
	\ifnum#3<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
		{\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
		}
		{\@xs@cutafteroccur@i{#1}{#2}{#3}}%
}
	
\long\def\@xs@cutafteroccur@i#1#2#3{%
	\def\@xs@reserved@D{#1}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#2}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\ifnum\decimalpart=\numexpr(#3)\relax % occurrence trouv\'ee ?
		\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter\def\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\@xs@argument@A}%
	\else
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		\global\let\groupID\@empty
	\fi
}

\@xs@newmacro*3\IfSubStr{1}{2}{0}{%
	\def\@xs@argument@A{#2}\def\@xs@argument@B{#3}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur
	\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter{\@xs@argument@B}{#1}%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*2\IfBeginWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@secondoftwo
		}
		{\def\@xs@next{%
			\expandafter\expandafter\expandafter\@xs@IfBeginWith@i\expandafter\expandafter\expandafter
				{\expandafter\@xs@argument@A\expandafter}\expandafter
				{\@xs@argument@B}}%
		}%
	\@xs@next
}

\long\def\@xs@IfBeginWith@i#1#2{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\expandafter\@xs@ifempty\expandafter{\@xs@argument@B}%
		{\let\@xs@next\@firstoftwo% #2 est vide, tous les tests sont pass\'es avec succ\`es : on renvoie #3
		}
		{\expandafter\@xs@ifempty\expandafter{\@xs@argument@A}%
			{\let\@xs@next\@secondoftwo% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
			\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
			\ifx\@xs@reserved@A\@xs@reserved@B% il y a \'egalit\'e...
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@B}\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A% on enl\`eve les 1ere unit\'es syntaxiques
				\def\@xs@next{% et on recommence avec ces arguments racourcis d'1 unit\'e syntaxique
					\expandafter\expandafter\expandafter\@xs@IfBeginWith@i
					\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}}%
			\else
				\let\@xs@next\@secondoftwo
			\fi
			}%
		}%
	\@xs@next
}

\@xs@newmacro*2\IfEndWith{}{2}{0}{%
	\def\@xs@argument@A{#1}\def\@xs@argument@B{#2}%
	\@xs@ifempty{#2}%
		{\let\@xs@reserved@A\@secondoftwo
		}
		{\expandafter\expandafter\expandafter\@xs@StrCount
			\expandafter\expandafter\expandafter{\expandafter\@xs@argument@A\expandafter}\expandafter
			{\@xs@argument@B}[\@xs@reserved@A]%
		\ifnum\@xs@reserved@A=\z@
			\let\@xs@reserved@A\@secondoftwo
		\else
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
				{\let\@xs@reserved@A\@firstoftwo}
				{\let\@xs@reserved@A\@secondoftwo}%
		\fi
		}%
	\@xs@reserved@A
}

\@xs@newmacro*4\IfSubStrBefore{1,1}{3}{0}{\@xs@IfSubStrBefore@i[#1]{#2}{#3}{#4}}

\def\@xs@IfSubStrBefore@i[#1,#2]#3#4#5{%
	\def\@xs@reserved@C{#3}%
	\ifx\@xs@exploregroups\relax% si on explore les groupes
		\let\@xs@reserved@B\@empty
		\let\@xs@nestlevel\z@
		\@xs@StrRemoveBraces@i% on retire les accolades
		\let\@xs@reserved@C\@xs@reserved@B
	\fi
	\def\@xs@reserved@A{#5}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#2}%
	\def\@xs@reserved@A{#4}%
	\expandafter\expandafter\expandafter\@xs@cutafteroccur\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@A}{#1}%
	\global\let\groupID\@empty
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		\@secondoftwo
		\@firstoftwo
}

\@xs@newmacro*4\IfSubStrBehind{1,1}{3}{0}{\@xs@IfSubStrBehind@i[#1]{#2}{#3}{#4}}

\long\def\@xs@IfSubStrBehind@i[#1,#2]#3#4#5{\@xs@IfSubStrBefore@i[#2,#1]{#3}{#5}{#4}}

\long\def\@xs@formatnumber#1#2{%
	\def\@xs@argument@A{#1}%
	\@xs@ifempty{#1}%
		{\def#2{0X}% si vide, renvoie 0X
		}
		{\@xs@returnfirstsyntaxunit{#1}\@xs@reserved@A
		\def\@xs@reserved@B{+}%
		\ifx\@xs@reserved@A\@xs@reserved@B
			\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@C
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			 	{\def#2{+0X}}
			 	{\expandafter\def\expandafter#2\expandafter{\expandafter+\expandafter0\@xs@reserved@C}}%
		\else
			\def\@xs@reserved@B{-}%
			\ifx\@xs@reserved@A\@xs@reserved@B
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@argument@A}\@xs@reserved@A
				\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
					{\def#2{-0X}}%
					{\expandafter\def\expandafter#2\expandafter{\expandafter-\expandafter0\@xs@reserved@A}}%
			\else
				\expandafter\def\expandafter#2\expandafter{\expandafter0\@xs@argument@A}%
			\fi
		\fi
		}%
}

\@xs@newmacro\IfInteger{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\let\@xs@after@intpart\@xs@afterinteger
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\ifnum\decimalpart=\z@
			\let\@xs@next\@firstoftwo% partie décimale constituée de 0 --> seul cas où on renvoie vrai
		\else
			\let\@xs@afterinteger\@xs@after@intpart
			\let\@xs@next\@secondoftwo
		\fi
	\else
		\let\@xs@afterinteger\@xs@after@intpart
		\let\@xs@next\@secondoftwo
	\fi
	\@xs@next
}

\@xs@newmacro\IfDecimal{}{1}{0}{%
	\@xs@formatnumber{#1}\@xs@reserved@A
	\decimalpart\z@
	\afterassignment\@xs@defafterinteger\integerpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@testdot\@xs@afterinteger\@xs@nil
	\ifx\@empty\@xs@afterdecimal
		\expandafter\@firstoftwo
	\else
		\expandafter\@secondoftwo
	\fi
}

\long\def\@xs@defafterinteger#1\relax\@xs@nil{\def\@xs@afterinteger{#1}}

\def\@xs@testdot{%
	\let\xs@decsep\@empty
	\@ifnextchar.%
		{\def\xs@decsep{.}\@xs@readdecimalpart}%
		{\@xs@testcomma}%
}

\def\@xs@testcomma{%
	\@ifnextchar,%
		{\def\xs@dessep{,}\@xs@readdecimalpart}%
		{\@xs@endnumber}%
}

\long\def\@xs@readdecimalpart#1#2\@xs@nil{%
	\ifx\@empty#2\@empty
		\def\@xs@reserved@A{0X}%
	\else
		\def\@xs@reserved@A{0#2}%
	\fi
	\afterassignment\@xs@defafterinteger\decimalpart\@xs@reserved@A\relax\@xs@nil
	\expandafter\@xs@endnumber\@xs@afterinteger\@xs@nil
}

\long\def\@xs@endnumber#1\@xs@nil{\def\@xs@afterdecimal{#1}}

% test d'\'egalit\'e sur des chaines (et des chaines contenant des nombres)
\long\def\@xs@IfStrEqFalse@i#1#2{\let\@xs@reserved@A\@secondoftwo}
\long\def\@xs@IfStrEqFalse@ii#1#2{% renvoie vrai si les 2 arg sont d\'ecimaux et s'ils sont \'egaux, faux sinon
	\@xs@IfDecimal{#1}%
		{\@xs@IfDecimal{#2}%
			{\ifdim#1pt=#2pt
				\let\@xs@reserved@A\@firstoftwo
			\else
				\let\@xs@reserved@A\@secondoftwo
			\fi% les 2 sont d\'ecimaux : on fait le test
			}%
			{\let\@xs@reserved@A\@secondoftwo}% un seul est d\'ecimal
		}%
		{\let\@xs@reserved@A\@secondoftwo}% #1 n'est pas d\'ecimal
}

\long\def\@xs@TestEqual#1#2{% teste si les 2 arguments sont \'egaux
	\def\@xs@reserved@A{#1}\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\let\@xs@reserved@A\@firstoftwo% \'egalit\'e parfaite des 2 chaines
	\else
		\expandafter\expandafter\expandafter\@xs@reserved@D\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@A\expandafter}\expandafter{\@xs@reserved@B}%
	\fi
	\@xs@reserved@A
}

\@xs@newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont \'egales
	\let\@xs@reserved@D\@xs@IfStrEqFalse@i
	\@xs@TestEqual{#1}{#2}%
}

\@xs@newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont \'egaux
	\let\@xs@reserved@D\@xs@IfStrEqFalse@ii
	\@xs@TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfStrEq*}\@xs@IfStrCase}%
		{\def\@xs@reserved@E{\IfStrEq}\@xs@IfStrCase}%
}

\long\def\@xs@IfStrCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\def\IfEqCase{%
	\@ifstar
		{\def\@xs@reserved@E{\IfEq*}\@xs@IfEqCase}%
		{\def\@xs@reserved@E{\IfEq}\@xs@IfEqCase}%
}

\long\def\@xs@IfEqCase#1#2{\@testopt{\@xs@IfStringCase{#1}{#2}}{}}

\long\def\@xs@IfStringCase#1#2[#3]{%
	\long\def\@xs@testcase##1##2##3\@xs@nil{% lit les 2 premieres unit\'es syntaxiques dans ##1 et ##2. Les autres dans ##3
		\@xs@reserved@E{#1}{##1}%
			{##2}% le test est positif, on ex\'ecute le code correspondant
			{\@xs@ifempty{##3}%
			 	{#3}% s'il n'y a plus de cas, on ex\'ecute le code <autres cas>
				{\@xs@testcase##3\@xs@nil}% sinon, on recommence avec ce qui reste
			 }%
	}%
	\@xs@testcase#2\@xs@nil
}

% Renvoie ce qui est \`a gauche de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBefore{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
}

% Renvoie ce qui est \`a droite de l'occurence n°#1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro*3\StrBehind{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n°#1 et n°#2
% des chaines #4 et #5 dans la chaine #3
\@xs@newmacro*4\StrBetween{1,1}{3}{1}{\@xs@StrBetween@i[#1]{#2}{#3}{#4}[#5]}

\long\def\@xs@StrBetween@i[#1,#2]#3#4#5[#6]{%
	\begingroup
		\noexploregroups
		\@xs@cutafteroccur{#3}{#5}{#2}%
		\expandafter\@xs@cutafteroccur\expandafter{\@xs@reserved@C}{#4}{#1}%
		\expandafter
	\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@E}{#6}%
	\global\let\groupID\@empty
}

\def\exploregroups{\let\@xs@exploregroups\relax}

\def\noexploregroups{\def\@xs@exploregroups{\let\@xs@toks0\relax}}

\def\saveexploremode{\let\@xs@saveexploremode\@xs@exploregroups}

\def\restoreexploremode{\let\@xs@exploregroups\@xs@saveexploremode}

% Remplace les #1 premi\`eres occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\@xs@newmacro\StrSubstitute{0}{3}{1}{%
	\def\@xs@reserved@D{#2}\let\@xs@reserved@C\@empty\def\@xs@reserved@E{#3}%
	\def\@xs@argument@C{#3}\def\@xs@argument@D{#4}%
	\decimalpart\z@
	\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum#1<\@ne
			\let\@xs@reserved@A\@xs@argument@D
		\else
			\ifnum\decimalpart>#1
				\let\@xs@reserved@A\@xs@argument@C
			\else
				\let\@xs@reserved@A\@xs@argument@D
			\fi
		\fi
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@A}%
		\@xs@read@reserved@D
	}%
	\@xs@ifempty{#3}%
		{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#5}%
		}
		{\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#5}%
		}%
}

% Supprime les #1 premi\`eres occurrences de #3 dans #2
\@xs@newmacro\StrDel{0}{2}{1}{\@xs@StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\@xs@exitallgroups{\ifnum\@xs@nestlevel>\z@\endgroup\expandafter\@xs@exitallgroups\fi}

% Compte combien d'unit\'es syntaxiques contient la chaine #1 ?
\@xs@newmacro\StrLen{}{1}{1}{%
	\def\@xs@reserved@C{#1}%
	\decimalpart\z@
	\let\@xs@nestlevel\z@
	\gdef\groupID{0}%
	\let\@xs@atbegingroup\relax
	\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
	\let\@xs@atnextsyntaxunit\relax
	\@xs@read@reserved@C
	\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n\'ecessaire pour trouver une unit\'e syntaxique derri\`ere
\def\@xs@continuetonext{%
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
		{\ifnum\@xs@nestlevel>\z@
			\expandafter\endgroup\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}% on concat\`ene
			\expandafter\expandafter\expandafter\@xs@continuetonext% on recommence
		\fi}
		\relax
}%

\def\@xs@manage@groupID{%
	\begingroup\def\@xs@reserved@A{0}%
	\ifx\@xs@reserved@A\groupID% si on arrive du groupe de niveau 0
		\endgroup
		\xdef\groupID{\number\integerpart}% on met simplement le niveau
	\else
		\endgroup
		\expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\groupID\expandafter\expandafter\expandafter{\expandafter\groupID\expandafter,\number\integerpart}%
	\fi
}

% Cette macro coupe la chaine #1 apr\`es l'unit\'e syntaxique n°#2
\def\StrSplit{%
	\@ifstar
		{\let\@xs@reserved@E\@xs@continuetonext\StrSpl@t}%
		{\let\@xs@reserved@E\relax\StrSpl@t}%
}

\@xs@newmacro\StrSpl@t{}{2}{0}{\@xs@StrSplit@i{#2}{#1}\@xs@StrSplit@ii}

% Cette macro interne coupe la chaine #2 apr\`es l'unit\'e syntaxique n°#1
% Le d\'ebut est assign\'e dans \@xs@reserved@B et la fin dans \@xs@reserved@C
\long\def\@xs@StrSplit@i#1#2{%
	\def\@xs@reserved@D{#1}%
	\def\@xs@reserved@C{#2}%
	\let\@xs@reserved@B\@empty
	\global\let\groupID\@empty
	\ifnum#1>\z@
		\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
			\@xs@read@reserved@C
		}%
		\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
		\def\@xs@atnextsyntaxunit{%
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\@xs@reserved@A}%
			\ifnum\decimalpart=\@xs@reserved@D\relax
				\ifx\@xs@reserved@C\@empty\@xs@reserved@E\fi
				\global\let\@xs@reserved@B\@xs@reserved@B
				\global\let\@xs@reserved@C\@xs@reserved@C
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
}

\def\@xs@StrSplit@ii#1#2{\let#1\@xs@reserved@B\let#2\@xs@reserved@C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA reçoit ce qui se trouve avant la n ème occurrence <motif> dans <texte>
% \macroB reçoit ce qui est après cette n ème occurrence
\@xs@newmacro*3\StrCut{1}{2}{0}{%
	\@xs@ifempty{#3}%
		{\global\let\groupID\@empty
		\let\@xs@reserved@C\@empty
		\let\@xs@reserved@E\@empty
		}
		{\ifnum#1<\@ne\expandafter\@firstoftwo\else\expandafter\@secondoftwo\fi
			{\@xs@StrCut@ii{#2}{#3}1}
			{\@xs@StrCut@ii{#2}{#3}{#1}}%
		}%
	\@xs@StrCut@iii
}

\long\def\@xs@StrCut@ii#1#2#3{%
	\def\@xs@reserved@D{#1}%
	\let\@xs@reserved@C\@empty
	\def\@xs@reserved@E{#2}%
	\decimalpart\z@\integerpart\z@
	\gdef\groupID{0}%
	\let\@xs@nestlevel\z@
	\def\@xs@atendofgroup{%
		\expandafter\endgroup
		\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
		\@xs@read@reserved@D
	}%
	\def\@xs@atoccurfound{%
		\ifnum\decimalpart=\numexpr(#3)\relax
			\global\let\@xs@reserved@D\@xs@reserved@D
			\global\let\@xs@reserved@C\@xs@reserved@C
			\@xs@exitallgroups
			\let\@xs@next\relax
		\else
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\@xs@reserved@E}%
			\let\@xs@next\@xs@read@reserved@D
		\fi
	}%
	\@xs@read@reserved@D
	\def\@xs@argument@A{#2}%
	\let\@xs@reserved@E\@xs@reserved@D
		\expandafter\expandafter\expandafter
	\def
		\expandafter\expandafter\expandafter
	\@xs@reserved@D
		\expandafter\expandafter\expandafter
	{\expandafter\@xs@reserved@C\@xs@argument@A}%
}

\long\def\@xs@StrCut@iii#1#2{\let#1\@xs@reserved@C\let#2\@xs@reserved@E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit\'es syntaxiques aux positions compris !
\@xs@newmacro\StrMid{}{3}{1}{%
	\begingroup
		\noexploregroups
		\let\@xs@reserved@E\relax
		\@xs@StrSplit@i{#3}{#1}%
		\edef\@xs@reserved@C{\number\numexpr#2-1}%
		\let\@xs@reserved@E\relax
		\expandafter\expandafter\expandafter\@xs@StrSplit@i\expandafter\expandafter\expandafter{\expandafter\@xs@reserved@C\expandafter}\expandafter{\@xs@reserved@B}%
	\expandafter\endgroup
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#4}%
	\global\let\groupID\@empty
}

% supprime #2 unit\'es syntaxiques \`a gauche dans la chaine #1
\@xs@newmacro\StrGobbleLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

% extrait de #1 la chaine \`a gauche de longueur #2
\@xs@newmacro\StrLeft{}{2}{1}{%
	\let\@xs@reserved@E\relax
	\@xs@StrSplit@i{#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% supprime #2 unit\'es syntaxiques \`a droite dans la chaine #1
\@xs@newmacro\StrGobbleRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% renvoie #2 unit\'es syntaxiques \`a la droite de la chaine #1
\@xs@newmacro\StrRight{}{2}{1}{%
	\@xs@StrLen{#1}[\@xs@reserved@D]%
	\let\@xs@reserved@E\relax
	\expandafter\@xs@StrSplit@i\expandafter{\number\numexpr\@xs@reserved@D-#2}{#1}%
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@C}{#3}%
}

\@xs@newmacro\StrChar{}{2}{1}{%
	\let\@xs@reserved@B\@empty
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\ifnum#2>\z@
		\def\groupID{0}\let\@xs@nestlevel\z@\integerpart\z@\decimalpart\z@
		\let\@xs@atbegingroup\relax
		\def\@xs@atendofgroup{\endgroup\@xs@read@reserved@C}%
		\def\@xs@atnextsyntaxunit{%
			\ifnum\decimalpart=\@xs@reserved@D% la n i\`eme US est atteinte ?
				\global\let\@xs@reserved@B\@xs@reserved@A% on capture l'US en cours qui est celle cherch\'ee
				\@xs@exitallgroups
				\let\@xs@next\relax
			\fi
		}%
		\@xs@read@reserved@C
	\fi
	\expandafter\@xs@ifempty\expandafter{\@xs@reserved@B}%
		{\global\let\groupID\@empty}
		\relax
	\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\@xs@newmacro\StrCount{}{2}{1}{%
	\def\@xs@reserved@D{#1}\def\@xs@reserved@E{#2}\let\@xs@reserved@C\@empty
	\@xs@ifempty{#2}%
		{\@xs@ReturnResult{0}{#3}}
		{\decimalpart\z@
		\integerpart\z@
		\gdef\groupID{0}%
		\let\@xs@nestlevel\z@
		\def\@xs@atendofgroup{%
			\expandafter\endgroup
			\expandafter\@xs@addtomacro\expandafter\@xs@reserved@C\expandafter{\expandafter{\@xs@reserved@C}}%
			\@xs@read@reserved@D
		}%
		\def\@xs@atoccurfound{\let\@xs@reserved@C\@empty\@xs@read@reserved@D}%
		\@xs@read@reserved@D
		\expandafter\@xs@ReturnResult\expandafter{\number\decimalpart}{#3}%
		}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\@xs@newmacro\StrPosition{1}{2}{1}{%
	\@xs@cutafteroccur{#2}{#3}{#1}%
	\let\@xs@reserved@E\groupID
	\ifx\@xs@reserved@C\@xs@reserved@D
		\@xs@ReturnResult{0}{#4}%
		\let\@xs@reserved@E\@empty
	\else
		\expandafter\@xs@StrLen\expandafter{\@xs@reserved@C}[\@xs@reserved@C]%
		\expandafter\@xs@ReturnResult\expandafter{\number\numexpr\@xs@reserved@C+1}{#4}%
	\fi
	\global\let\groupID\@xs@reserved@E
}

\def\comparestrict{\let\@xs@comparecoeff\@ne}

\def\comparenormal{\let\@xs@comparecoeff\z@}

\def\savecomparemode{\let\@xs@saved@comparecoeff\@xs@comparecoeff}

\def\restorecomparemode{\let\@xs@comparecoeff\@xs@saved@comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont \'egaux et renvoie la
% position de la premiere unit\'e syntaxiques diff\'erente sinon
\@xs@newmacro*2\StrCompare{}{2}{1}{%
	\def\@xs@reserved@A{#1}%
	\def\@xs@reserved@B{#2}%
	\ifx\@xs@reserved@B\@xs@reserved@A
		\@xs@ReturnResult{0}{#3}%
	\else
		\def\@xs@next{\@xs@StrCompare@i{#1}{#2}{#3}}%
		\expandafter\@xs@next
	\fi
}

\long\def\@xs@StrCompare@i#1#2#3{%
	\def\@xs@StrCompare@iii##1{%
		\let\@xs@reserved@A\@empty
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@reserved@A{*\@xs@comparecoeff}}%
			{\expandafter\@xs@ifempty\expandafter{\@xs@reserved@D}%
				{\def\@xs@reserved@A{*\@xs@comparecoeff}}
				\relax
			}%
		\def\@xs@next{%
			\expandafter\@xs@ReturnResult\expandafter
			{\number\numexpr##1\@xs@reserved@A\relax}{#3}%
		}%
	}%
	\def\@xs@StrCompare@ii##1{% ##1 est la position
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@A
		\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@B
		\ifx\@xs@reserved@B\@xs@reserved@A
			\expandafter\@xs@ifempty\expandafter{\@xs@reserved@A}%
				{\@xs@StrCompare@iii{##1}% les 2 unit\'es syntaxiques sont \'egales, on renvoie la position
				}
				{\def\@xs@next{\expandafter\@xs@StrCompare@ii\expandafter{\number\numexpr##1+1}}% les 2 unit\'es syntaxiques sont \'egales et non vides, on recommence
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@D}\@xs@reserved@D
				}%
		\else% les 2 unit\'es syntaxiques sont diff\'erentes : on renvoie la position
			\@xs@StrCompare@iii{##1}%
		\fi
		\@xs@next
	}%
	\def\@xs@reserved@C{#1}\def\@xs@reserved@D{#2}%
	\@xs@StrCompare@ii1%
}

\@xs@newmacro\StrFindGroup{}{2}{1}{%
	\def\@xs@reserved@A{#2}\def\@xs@reserved@B{0}%
	\ifx\@xs@reserved@A\@xs@reserved@B
		\def\@xs@next{\@xs@ReturnResult{{#1}}{#3}}%
	\else
		\def\@xs@next{\@xs@StrFindGroup@i{#1}{#2}[#3]}%
	\fi
	\@xs@next
}

\long\def\@xs@StrFindGroup@i#1#2[#3]{%
	\def\@xs@StrFindGroup@ii{%
		\expandafter\@xs@ifempty\expandafter{\@xs@reserved@C}%
			{\def\@xs@next{\@xs@ReturnResult{}{#3}}% s'il ne reste plus rien, on renvoie vide
			}
			{\expandafter\@xs@returnfirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@D
			\ifx\bgroup\@xs@toks% si la 1\`ere unit\'e syntaxique est un groupe explicite
				\advance\decimalpart\@ne% on augmente le compteur
				\ifnum\decimalpart=\@xs@reserved@A% on est au groupe cherch\'e lors de la profondeur courante ?
					\ifx\@empty\@xs@reserved@B% on est \`a la profondeur maximale ?
						\def\@xs@next{\expandafter\@xs@ReturnResult\expandafter{\@xs@reserved@D}{#3}}% on renvoie ce groupe
					\else% sinon
						\expandafter\def\expandafter\@xs@next\expandafter{\expandafter\@xs@StrFindGroup@i\@xs@reserved@D}% on recommence avec ce groupe
						\expandafter\@xs@addtomacro\expandafter\@xs@next\expandafter{\expandafter{\@xs@reserved@B}[#3]}% et les profondeurs de recherche restantes
					\fi
				\else
					\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
					\let\@xs@next\@xs@StrFindGroup@ii
				\fi
			\else
				\expandafter\@xs@removefirstsyntaxunit\expandafter{\@xs@reserved@C}\@xs@reserved@C
				\let\@xs@next\@xs@StrFindGroup@ii
			\fi
			}%
		\@xs@next
	}%
	\@xs@extractgroupnumber{#2}\@xs@reserved@A\@xs@reserved@B
	\decimalpart\z@
	\ifnum\@xs@reserved@A>\z@\def\@xs@reserved@C{#1}\else\let\@xs@reserved@C\@empty\fi
	\@xs@StrFindGroup@ii
}

\def\@xs@extractgroupnumber#1#2#3{%
	\def\@xs@extractgroupnumber@i##1,##2\@xs@nil{\def#2{##1}\def#3{##2}}%
	\@xs@extractgroupnumber@i#1,\@xs@nil
	\ifx\@empty#3\else\@xs@extractgroupnumber@i#1\@xs@nil\fi
}

\def\expandingroups{\let\@xs@expandingroups\exploregroups}

\def\noexpandingroups{\let\@xs@expandingroups\noexploregroups}

\def\StrExpand{\@testopt{\@xs@StrExpand}{1}}
\long\def\@xs@StrExpand[#1]#2#3{%
	\begingroup
		\@xs@expandingroups
		\ifnum#1>\z@
			\integerpart#1\relax
			\decimalpart\z@
			\gdef\groupID{0}%
			\let\@xs@nestlevel\z@
			\def\@xs@atendofgroup{%
				\expandafter\endgroup
				\expandafter\@xs@addtomacro\expandafter\@xs@reserved@B\expandafter{\expandafter{\@xs@reserved@B}}%
				\@xs@read@reserved@C
			}%
			\def\@xs@atbegingroup{\let\@xs@reserved@B\@empty}%
			\def\@xs@atnextsyntaxunit{%
				\expandafter\expandafter\expandafter\@xs@addtomacro
				\expandafter\expandafter\expandafter\@xs@reserved@B
				\expandafter\expandafter\expandafter{\@xs@reserved@A}%
			}%
			\def\@xs@reserved@C{#2}%
			\@xs@StrExpand@i{#1}% Appel de la macro r\'ecursive
		\else
			\def\@xs@reserved@B{#2}%
		\fi
		\global\let\@xs@reserved@B\@xs@reserved@B
	\endgroup
	\let#3\@xs@reserved@B
	\global\let\groupID\@empty
}

\long\def\@xs@StrExpand@i#1{%
	\ifnum#1>\z@
		\let\@xs@reserved@B\@empty
		\@xs@read@reserved@C
		\let\@xs@reserved@C\@xs@reserved@B
		\def\@xs@reserved@A{\expandafter\@xs@StrExpand@i\expandafter{\number\numexpr#1-1}}%
	\else
		\let\@xs@reserved@A\relax
	\fi
	\@xs@reserved@A
}

\def\scancs{\@testopt{\@xs@scancs}{1}}
\long\def\@xs@scancs[#1]#2#3{%
	\@xs@StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

% Restaure le code de @
\catcode`\@=\CurrentAtCatcode\relax

% D\'efinit le d\'elimiteur verb
% d\'efinit les diff\'erents modes et les m\'emorise
\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput
%
% Historique
%------------------------------------------------------------------------------
%% v1.0    4/7/2008 : - Package achev\'e.
%          7/7/2008 : - Package publi\'e sur CTAN.
%------------------------------------------------------------------------------
% v1.1    15/8/2008
%   - Le package ne n\'ecessite plus LaTeX et est d\'esormais utilisable sous
%     Plain eTeX.
%   - Ajout des macros \IfInteger et \IfDecimal.
%     Pour cette derni\`ere, la partie enti\`ere et la partie d\'ecimale sont
%     r\'ecup\'erables dans les compteurs \integerpart et \decimalpart. Ce
%     qu'il reste apr\`es qu'un caract\`ere non attendu soit rencontr\'e est
%     dispo dans \@xs@remainafterdecimal
%   - Correction d'un bug dans \tokenize :
%        suppression de l'expansion avec \normalexpandarg pour \'eviter le bug
%        avec les lettres accentu\'ees dans l'exemple : \tokenize\aa{\'e\`u}
%   - Am\'elioration du code de la plupart des macros.
%   - \'Ecriture d'une routine \@xs@newmacro d\'efinissant les  macros.
%   - Suppression de tous les compteurs grace \`a \numexpr.
%   - Nouvelles fonctionnalit\'es internes dans :
%      \IfSubStr
%        ajout des chaines se trouvant avant et apr\`es l'occurrence test\'ee
%        dans les sc \@xs@behind@IfSubStr et \@xs@before@IfSubStr
%      \StrCount
%        a) ajout de ce qui se trouve apr\`es la derni\`ere occurrence dans la
%           sc \@xs@StrCount@afterlastocccur
%        b) la macro ne d\'epend plus d'aucune autre
%------------------------------------------------------------------------------
% v1.2    23/8/2008
%   - Am\'elioration du code de \StrMid \StrGobbleLeft, \StrLeft,
%     \StrGobbleRight et \StrRight \`a l'aide de la nouvelle macro
%     \@xs@StrSplit@i
%   - Nouveau test \IfStrEq qui compare 2 chaines
%   - Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
%     contiennent un nombre)
%   - Correction d'un bug dans \@xs@formatnumber. La macro n'envisageait pas le
%     cas o\`u son argument \'etait vide ce qui faiasait planter
%     \IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
%------------------------------------------------------------------------------
% v1.3    21/9/2008
%  - Am\'elioration du code, mise en place de r\'ecursivit\'es terminales dans
%    toutes les macros r\'ecursives, simplification de \@xs@TestEqual en
%    utilisant \ifx
%  - Nouvelles macros \IfStrEqCase et \IfEqCase
%      Teste si une chaîne est \'egale \`a plusieurs cha\^ines donn\'ee et
%      ex\'ecute un code sp\'ecifique
%  - Cr\'eation de la macro publique \StrSplit
%      Coupe la chaine en 2 \`a une position donn\'ee
%  - Nouvelle macro \StrCompare
%      Compare 2 chaînes et renvoie la position du 1er caract\`ere diff\'erent.
%      Renvoie 0 si elles sont \'egales.
%------------------------------------------------------------------------------
% v1.3a   29/9/2008
%  - Correction d'un bug : \expandafter#1
%    dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
%    nombre > 9 !
%  - R\'e \'ecriture de \@xs@returnfirstsyntaxunit et \@gobble qui
%    deviennent purement d\'eveloppables.
%  - R\'e \'ecriture de \StrLen
%  - Nouvelle macro interne \@xs@cutafteroccur
%      Coupe la chaine apr\`es la ni\`eme occurrence d'une sous chaine.
%  - Code am\'elior\'e de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
%    \StrGobbleRight grace \`a \@xs@cutafteroccur
%------------------------------------------------------------------------------
% v1.4   4/11/2008
%  - xstring traite ses arguments par unit\'e syntaxique, et donc toutes les
%    macros internes ont \'et\'e r\'e-\'ecrites \`a cette fin.
%  - Le manuel a \'et\'e r\'e-\'ecrit, rendu plus clair et mieux structur\'e.
%  - Nouvelle fonctionnalit\'e : \expandarg
%      le 1er lex\`eme de chaque argument est 1-d\'evelopp\'e avant que la
%      macro ne soit appel\'ee. Si un argument comporte plus qu'1 lex\`eme,
%      il faut passer par \scancs*[1] pour 1-d\'evelopper toutes les unit\'es
%      syntaxiques.
%  - Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
%    d\'efaut dans \StrSubstitute et \StrDel
%  - Coh\'erence dans les nom des s\'equences de contr\^oles temporaires qui
%    sont d\'esormais : \@xs@reserved@A \`a \@xs@reserved@E
%------------------------------------------------------------------------------
% v1.4a  12/11/2008
%  - Correction d'un bug dans \@xs@StrSplit dans le cas o\`u l'argument
%     num\'erique est <1 : la 1ere coupure doit être vide et le seconde doit
%     être \'egale \`a l'argument.
%------------------------------------------------------------------------------
% v1.4b  16/11/2008
%  - Correction de 2 bugs dans \@xs@returnfirstsyntaxunit
%------------------------------------------------------------------------------
% v1.5   31/12/2008
%  - Nouvelles fonctionnalit\'es dans la recherche de groupes par un
%    identificateur caract\'erisant leur imbrication. Impl\'ementation de :
%      1) \StrFindGroup
%      2) \groupID
%  - Ajout des nouvelles macros g\'en\'eriques \@xs@read@reserved@C et
%    \@xs@read@reserved@D
%  - Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
%    que \truc contenait «a{a}».
%  - Correction d'un bug dans \@xs@newmacro : l'argument optionnel \'etait
%    d\'etok\'enis\'e \`a tort dans les macros \'etoil\'ees.
%  - Dans \@xs@newmacro, on doit choisir le num\'ero du dernier argument devant
%    être d\'etok\'enis\'e dans le cas d'une macro \'etoil\'ee (sachant que
%     l'argument optionnel ne l'est jamais)
%------------------------------------------------------------------------------
% v1.5a  09/2/2009
%  - Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
%    indépendante du mode d'exploration et dispose de ses propres commandes
%    d'exploration : \expandingroups et \noexpandingroups
%  - R\'e-\'ecriture de \scancs, qui devient triviale puisque d\'ependant de
%    \StrExpand. Il n'y a plus de version \'étoil\'ee et d\'esormais, \scancs
%    est sensible au mode d'exploration.
%  - Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
%  - Correction de bugs : mettre \let\@xs@reserved@E\relax avant d'appeler
%    \@xs@StrSplit@i
%  - Suppression des messages d'erreur, de warning et d'info. xstring devient
%    donc silencieux ;)
%  - Passage de 3 \'a 2 compteurs
%  - Le manuel est d\'esormais plus color\'e, en esp\'erant qu'il sera un peu
%    plus agr\'eable \`a lire !
%------------------------------------------------------------------------------
% v1.5b  13/3/2009
%  - Modification d'un grand nombre de macros de telle sorte que vraiment
%    n'importe quel code peut d\'esormais \^etre plac\'e dans les arguments des
%    macros (comme par exemple des \if, \ifx ou autre, m\^eme sans leur \fi, ce
%    qui n'\'etait pas possible jusqu'alors)
%------------------------------------------------------------------------------
% v1.5c  05/6/2009
%  - Correction d'un bug dans \IfBeginWith : il faut appeler
%    \@xs@returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
%    non pas l'inverse pour que \@xs@toks reflète ce qui se trouve dans #1
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit au cas où #1 commence
%    par un espace : mettre \@xs@toks à 0
%  - Correction d'un bug dans \@xs@returnfirstsyntaxunit :
%    \@xs@returnfirstsyntaxunit{{}}\truc
%    faisait que \truc se développait en un espace.
%  - Correction d'un bug dans \@xs@removefirstsyntaxunit où le cas
%    \@xs@removefirstsyntaxunit{ {b}}\truc
%    donnait \truc se développant en «b» au lieu de «{b}».
%------------------------------------------------------------------------------
% v1.5d  28/3/2010
%  - Correction d'un bug dans \IfInteger : \@xs@afterinteger ne donnait pas le
%    bon r\'esultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
%  - \xs@formatnumber ne detokenize plus ses arguments (que m'est-il pass\'e
%    par la t\^ete pour que je code un truc comme ca ?), et donc
%    \@xs@afterinteger et \@xs@afterdecimal ont des tokens ayant le bon
%    catcode
%------------------------------------------------------------------------------
% v1.6  24/10/2012
%  - Correction d'un bug dans \@xs@cutafteroccur au cas o\`u #3<1
%  - \IfDecimal ne \detokenize plus l'argument.
%  - Nouvelle version de \tokenize qui enlevait les accolades si son argument
%    \'etait entre accolades
%  - Nouvelle macro \StrCut
%  - \@xs@cutafteroccur@i ne produit plus d'espace indésirable si #3 était
%    évalué par \numexpr
%------------------------------------------------------------------------------
% v1.7  13/1/2013
%  - Correction d'un manque de rigueur dans les assignations concernant
%    \groupID : elles sont toutes globales d\'esormais
%  - Les macros de xstring sont \long
%------------------------------------------------------------------------------
% v1.7a 28/2/2013
%  - Correction d'un espace parasite dans \@xs@removefirstsyntaxunit
%------------------------------------------------------------------------------
% v1.7b 29/7/2013
%  - La date contenue dans \xstringdate est désormais conforme
%------------------------------------------------------------------------------
% v1.7c 13/10/2013 
%  - les macros impliquées dans \IfStrCase et \IfStrEqCase sont désormais \long
